Learning Monocular Depth in Dynamic Environment via Context-aware Temporal Attention

The monocular depth estimation task has recently revealed encouraging prospects, especially for the autonomous driving task. To tackle the ill-posed problem of 3D geometric reasoning from 2D monocular images, multi-frame monocular methods are developed to leverage the perspective correlation information from sequential temporal frames. However, moving objects such as cars and trains usually violate the static scene assumption, leading to feature inconsistency deviation and misaligned cost values, which would mislead the optimization algorithm. In this work, we present CTA-Depth, a Context-aware Temporal Attention guided network for multi-frame monocular Depth estimation. Specifically, we first apply a multi-level attention enhancement module to integrate multi-level image features to obtain an initial depth and pose estimation. Then the proposed CTA-Refiner is adopted to alternatively optimize the depth and pose. During the refinement process, context-aware temporal attention (CTA) is developed to capture the global temporal-context correlations to maintain the feature consistency and estimation integrity of moving objects. In particular, we propose a long-range geometry embedding (LGE) module to produce a long-range temporal geometry prior. Our approach achieves significant improvements over state-of-the-art approaches on three benchmark datasets.

==> conclusion.tex <==
% \section{Conclusion}
% In this work, we propose CTA-Depth, a context-aware temporal attention guided network for supervised multi-frame monocular depth and pose estimation, especially for the dynamic object targets.
% We discard the explicit object motion module and inherently boost the long-range multi-frame context-temporal feature integration.
% Firstly, we utilize the multi-level attention enhancement (MAE) module to realize the reliable initial estimation, concerning about the distant small targets.
% Then we adopt the refiner CTA-Refiner to iteratively optimize our predictions, where we propose depth-pose context-aware temporal attention (CTA) to keep sufficient context-temporal correlations and feature consistency for moving objects, and the long-range geometry embedding (LGE) to expand the temporal interest field.
% Extensive experiments on three datasets demonstrate the effectiveness and superiority of our approach over state-of-the-arts.

% \if 0
\section{Conclusion}

In this work, we present a novel CTA-Depth for multi-frame monocular depth estimation. To resolve the ambiguity caused by challenging dynamic scenes with moving objects, we propose the CTA-Refiner by designing context-aware temporal attention to implicitly leverage temporal information and model image self-similarities. In addition, we develop a novel long-range geometry embedding module to efficiently inject our refiner with geometry reasoning among the long-range temporal frames.
Furthermore, we build a multi-level encoder-decoder network with the attention-enhanced predictor to obtain features with both global and local attentions. We achieve state-of-the-art performances on three challenging monocular depth estimation benchmarks.
In the future, we would like to employ our multi-frame association mechanism in relevant tasks such as 3D object detection.

%  and messy environments.  

% In the future, we would like to investigate the possibility of combining our proposed context-aware temporal attention based refinement network in other monocular depth estimation methods (including self-supervised methods), as well as the novel context-aware temporal attention mechanisms extended to other dynamic perception tasks.

% In the future, we would also like to employ our predicted depth maps to various downstream tasks, such as 3D object detection,3D scene reconstruction, etc.
%Our TransOpt achieves the state-of-the-art across all metrics on KITTI, Virtual KITTI 2, and NuScenes datasets. In future work, we would like to investigate the insight of our novel attention mechanism and extend it into other dynamic system. 
%Further, we would also like to extend our TransOpt module for other optimizer-based method and tasks.

% \fi

==> experiment.tex <==
\section{Experiments and Results}
\label{sec:experiments}

\begin{table*}[t]
	\centering
% 	Note that, "M→O" means monocular multiple frame images are used in training while only single frame image is used for inference. and "MF" means monocular multi-frames are both used in traning and inference.“SF” means single frame.
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{@{}lccccccccccc@{}}
			\toprule
			Method            & Cap    & Input          & GT type & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$   & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ \\ \midrule
			PackNet-SfM \cite{guizilini20203d}       & 0-80m     & M$\to${S}         &Velodyne& 0.090& 0.618& 4.220& 0.179& 0.893& 0.962& 0.983         \\
			DRO \cite{gu2023dro}                & 0-80m       & Multi-Frame                &Velodyne& 0.073& 0.528& 3.888& 0.163& 0.924& 0.969& 0.984         \\
			CTA-Depth (ours)            &         0-80m      & Multi-Frame               & Velodyne         &   0.071      &     0.496   &   3.598    &   0.143    &   0.931    &    0.975     &  0.989      \\
			\midrule
			BTS \cite{lee2019big}              & 0-80m     & Single-Frame         & Improved & 0.059 & 0.241  & 2.756 & 0.096 & 0.956 & 0.993   & 0.998   \\
			GLPDepth \cite{kim2022global}    & 0-80m        & Single-Frame                &Improved& 0.057& \multicolumn{1}{c}{--}& 2.297& 0.086& 0.967& 0.996& 0.999 \\
			PackNet-SfM \cite{guizilini20203d}       & 0-80m    & M$\to${S}                & Improved & 0.064 & 0.300  & 3.089 & 0.108 & 0.943 & 0.989   & 0.997   \\
			\midrule
			BANet \cite{tang2018ba}   & 0-80m & Multi-Frame & Improved & 0.083 & \multicolumn{1}{c}{--} & 3.640 & 0.134 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}  \\
			DeepV2D(2-view) \cite{teed2019deepv2d}    & 0-80m    & Multi-Frame                    &Improved& 0.064& 0.350& 2.946& 0.120& 0.946& 0.982& 0.991         \\
			DRO \cite{gu2023dro}         & 0-80m     & Multi-Frame                   &Improved& 0.047& 0.199& 2.629& 0.082& 0.970& 0.994& 0.998        \\
                \textbf{CTA-Depth}            &         0-80m        & Multi-Frame             &   Improved       & \textbf{0.038}       &    \textbf{0.145}  &   \textbf{2.224}    &  \textbf{0.069}     &   \textbf{0.978}    &    \textbf{0.996}     & \textbf{0.999}      \\
			% \textbf{CTA-Depth}            &         0-80m        & Multi-Frame             &   Improved       & 0.038       &    0.157  &   2.288    &  0.071     &   0.977    &    \textbf{0.996}     & \textbf{0.999}      \\
			% \textbf{CTA-Depth(L)}            &         0-80m        & Multi-Frame             &   Improved       &  \textbf{0.037}       &     \textbf{0.139}   &   \textbf{2.191}    &  \textbf{0.068}     &   \textbf{0.980}    &    \textbf{0.996}     &   \textbf{0.999}      \\
			% \midrule
			% % ResNet-18 + TransOpt,Swin-L + TransOpt	
   %              \textit{Improvement v.s. Multi-Frame Baseline} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}& \multicolumn{1}{c}{--} & \textcolor{blue}{19.1$\%$} $\uparrow$ &  \textcolor{blue} {27.1$\%$} $\uparrow$ &  \textcolor{blue}{15.4$\%$} $\uparrow$ &  \textcolor{blue}{15.8$\%$} $\uparrow$ &  \textcolor{blue}{0.8$\%$} $\uparrow$ &  \textcolor{blue}{0.2$\%$} $\uparrow$& \multicolumn{1}{c}{--}\\
			% \textit{Improvement v.s. Multi-Frame Baseline} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}& \multicolumn{1}{c}{--} & \textcolor{blue}{21.3$\%$} $\uparrow$ &  \textcolor{blue} {30.2$\%$} $\uparrow$ &  \textcolor{blue}{16.7$\%$} $\uparrow$ &  \textcolor{blue}{17.1$\%$} $\uparrow$ &  \textcolor{blue}{1.0$\%$} $\uparrow$ &  \textcolor{blue}{0.2$\%$} $\uparrow$& \multicolumn{1}{c}{--}\\
			\bottomrule
		\end{tabular}%
    }
    \caption{Quantitative results of supervised monocular depth estimation methods on the KITTI Eigen split. Note that the seven widely-used metrics are calculated strictly following the baseline \protect\cite{gu2023dro} and ground-truth median scaling is applied.
    ``M→S" means monocular multiple frame images are used in training while only a single frame image is used for inference. 
    We utilize bold to highlight the best results and color the multi-frame baseline results and our performance gain over them in blue.}
    \label{table_kitti_1}
    \vspace*{-2mm}
\end{table*}
% We utilize bold to highlight the best results, and color the previous-best ones and our performance gain over them in blue.
% \toprule
% 			Method            & Cap    & Input          & GT type & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$   & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ \\ \midrule
% 			PackNet-SfM\cite{guizilini20203d}       & 0-80m     & M$\to${O}         &Velodyne& 0.090& 0.618& 4.220& 0.179& 0.893& 0.962& 0.983         \\
% 			DRO\cite{gu2023dro}                & 0-80m       & Multi-Frame                &Velodyne& 0.073& 0.528& 3.888& 0.163& 0.924& 0.969& 0.984         \\
% 			CTA-Depth (ours)            &         0-80m      & Multi-Frame               & Velodyne         &   0.071      &     0.496   &   3.598    &   0.143    &   0.931    &    0.975     &  0.989      \\
% 			\midrule
% 			BANet\cite{tang2018ba}   & 0-80m & Multi-Frame & Improved & 0.083 & \multicolumn{1}{c}{--} & 3.640 & 0.134 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}  \\
% 			DeepV2D(2-view)\cite{teed2019deepv2d}    & 0-80m    & Multi-Frame                    &Improved& 0.064& 0.350& 2.946& 0.120& 0.946& 0.982& 0.991         \\
% 			PackNet-Sfm\cite{guizilini20203d}       & 0-80m    & M$\to${O}                & Improved & 0.064 & 0.300  & 3.089 & 0.108 & 0.943 & 0.989   & 0.997   \\
% 			BTS\cite{lee2019big}              & 0-80m     & Single-Frame         & Improved & 0.059 & 0.241  & 2.756 & 0.096 & 0.956 & 0.993   & 0.998   \\
% 			DRO\cite{gu2023dro}               & 0-80m     & Multi-Frame                   &Improved& \textcolor{blue} {0.047}& \textcolor{blue} {0.199}& 2.629& \textcolor{blue} {0.082}& \textcolor{blue} {0.970}& 0.994& 0.998        \\
% 			GLPDepth\cite{kim2022global}    & 0-80m        & Single-Frame                &Improved& 0.057& \multicolumn{1}{c}{--}& \textcolor{blue} {2.297}& 0.086& 0.967& \textcolor{blue} {0.996}& \textcolor{blue} {0.999}         \\
% 			CTA-Depth            &         0-80m        & Multi-Frame             &   Improved       & 0.040       &    0.157  &   2.288    &  0.071     &   0.977    &    \textbf{0.996}     & \textbf{0.999}      \\
% 			\textbf{CTA-Depth(L)}            &         0-80m        & Multi-Frame             &   Improved       &  \textbf{0.037}       &     \textbf{0.139}   &   \textbf{2.191}    &  \textbf{0.068}     &   \textbf{0.980}    &    \textbf{0.996}     &   \textbf{0.999}      \\
% 			\midrule
% 			% ResNet-18 + TransOpt,Swin-L + TransOpt	
% 			\textit{Improvement v.s. our Baseline} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \textcolor{blue}{21.3$\%$} $\uparrow$ &  \textcolor{blue} {30.2$\%$} $\uparrow$ &  \textcolor{blue}{16.7$\%$} $\uparrow$ &  \textcolor{blue}{17.1$\%$} $\uparrow$ &  \textcolor{blue}{1.0$\%$} $\uparrow$ &  \textcolor{blue}{0.2$\%$} $\uparrow$& \multicolumn{1}{c}{--}\\
% 			\bottomrule
% \begin{tabular}{@{}lcccccccccc@{}}
% 			\toprule
% 			Method            & Input              & GT type & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$   & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ \\ \midrule
% 			PackNet-SfM\cite{guizilini20203d}       & M$\to${O}              &Velodyne& 0.090& 0.618& 4.220& 0.179& 0.893& 0.962& 0.983         \\
% 			DRO\cite{gu2023dro}                & MF                        &Velodyne& 0.073& 0.528& 3.888& 0.163& 0.924& 0.969& 0.984         \\
% 			CTA-Depth (ours)            &         MF                     & Velodyne         &   0.071      &     0.496   &   3.598    &   0.143    &   0.931    &    0.975     &  0.989      \\
% 			\midrule
% 			BANet\cite{tang2018ba}   & MF  & Improved & 0.083 & \multicolumn{1}{c}{--} & 3.640 & 0.134 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}  \\
% 			DeepV2D(2-view)\cite{teed2019deepv2d}    & MF                        &Improved& 0.064& 0.350& 2.946& 0.120& 0.946& 0.982& 0.991         \\
% 			PackNet-Sfm\cite{guizilini20203d}       & M$\to${O}                    & Improved & 0.064 & 0.300  & 3.089 & 0.108 & 0.943 & 0.989   & 0.997   \\
% 			BTS\cite{lee2019big}              &  MF              & Improved & 0.059 & 0.241  & 2.756 & 0.096 & 0.956 & 0.993   & 0.998   \\
% 			DRO\cite{gu2023dro}                & MF                        &Improved& \textcolor{blue} {0.047}& \textcolor{blue} {0.199}& 2.629& \textcolor{blue} {0.082}& \textcolor{blue} {0.970}& 0.994& 0.998        \\
% 			GLPDepth\cite{kim2022global}    & MF                        &Improved& 0.057& \multicolumn{1}{c}{--}& \textcolor{blue} {2.297}& 0.086& 0.967& \textcolor{blue} {0.996}& \textcolor{blue} {0.999}         \\
% 			CTA-Depth            &         MF                     &   Improved       & 0.040       &    0.157  &   2.288    &  0.071     &   0.977    &    \textbf{0.996}     & \textbf{0.999}      \\
% 			\textbf{CTA-Depth(L)}            &         MF                     &   Improved       &  \textbf{0.037}       &     \textbf{0.139}   &   \textbf{2.191}    &  \textbf{0.068}     &   \textbf{0.980}    &    \textbf{0.996}     &   \textbf{0.999}      \\
% 			\midrule
% 			% ResNet-18 + TransOpt,Swin-L + TransOpt	
% 			\textit{Improvement v.s. our Baseline} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \textcolor{blue}{21.3$\%$} $\uparrow$ &  \textcolor{blue} {30.2$\%$} $\uparrow$ &  \textcolor{blue}{16.7$\%$} $\uparrow$ &  \textcolor{blue}{17.1$\%$} $\uparrow$ &  \textcolor{blue}{1.0$\%$} $\uparrow$ &  \textcolor{blue}{0.2$\%$} $\uparrow$& \multicolumn{1}{c}{--}\\
% 			\bottomrule
% 		\end{tabular}%
		
% 	}
% % \vspace*{-1mm}
% \end{table*}

% \begin{table*}[t]
%     \centering
% 	\footnotesize
% 	\setlength{\tabcolsep}{3.5pt}
% 	% table caption is above the table
% 	\caption{Quantitative results on KITTI Eigen split. Seven widely-used metrics are reported. Note that, the metrics is calculated following AdaBins\cite{bhat2021adabins}. “Abs Rel” error is the main ranking metric. “*” means using additional data for training. Highlighting: \textcolor{blue}{previous-best}, \textbf{best},  \textcolor{blue}{our improvement}.}
% 	\label{table_kitti_2}       % Give a unique label
% 	% For LaTeX tables use
% % 	\vspace{-0.5em}
% 	\centering
% 	\resizebox{\textwidth}{!}
% 	{%
% 		\begin{tabular}{lcccccccc}
% 			\toprule
% 			Method   & Reference  & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$ & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ \\ 
% 			\midrule
% 			Xu et al.\cite{xu2018structured} & CVPR 2018 & 0.122 & 0.897 & 4.677 & \multicolumn{1}{c}{--} &  0.818 &  0.954 & 0.985\\
% 			DORN\cite{fu2018deep} & CVPR 2018 & 0.072 & 0.307 & 2.727 & 0.120 & 0.932 & 0.984 & 0.995\\
% 			Yin et al.\cite{yin2019enforcing} & ICCV 2019 & 0.072 & \multicolumn{1}{c}{--} &  3.258 &  0.117 &  0.938 &  0.990 & 0.998\\
% 			% 		BTS\cite{lee2019big} & \multicolumn{1}{c}{--} & 0.059 & 0.245 &  2.756 &  0.096 &  0.956 &  0.993 & 0.998\\ 
% 			PackNet-SAN\cite{guizilini2021sparse} & CVPR 2021 & 0.062 & \multicolumn{1}{c}{--} &  2.888 &  \multicolumn{1}{c}{--} &  0.955 &  \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}\\
% 			DPT*\cite{ranftl2021vision} & ICCV 2021 & 0.062 & \multicolumn{1}{c}{--} &  2.573 &  0.092 &  0.959 &
% 			\textcolor{blue}{0.995} & \textcolor{blue}{0.999}\\
% 			PWA\cite{lee2021patch} & AAAI 2021 & 0.060 & 0.221 &  2.604 &  0.093 &  0.958 &  0.994 & \textcolor{blue}{0.999}\\
% 			AdaBins\cite{bhat2021adabins} & CVPR 2021 & 0.058 & \textcolor{blue}{0.190} &  \textcolor{blue}{2.360} &  \textcolor{blue}{0.088} &  \textcolor{blue}{0.964} &
% 			\textcolor{blue}{0.995} &
% 			\textcolor{blue}{0.999}\\
% 			\lzz{DRO\cite{patil2022p3depth} & \multicolumn{1}{c}{--} & \textcolor{blue}{0.052} & 0.270 &  2.842 &  0.103 &  0.953 &  0.993 & 0.998}\\
% 			NeWCRFs\cite{patil2022p3depth} & CVPR 2022 & 0.052 & 0.155 &  2.129 &  0.079 &  0.974 &  0.997 & 0.999\\
% 			P3Depth\cite{patil2022p3depth} & CVPR 2022 & 0.071 & 0.270 &  2.842 &  0.103 &  0.953 &  0.993 & 0.998\\
% 			TA-Opt& \multicolumn{1}{c}{--} &  0.047 & 0.174 &  2.352 & 0.077 &  0.974 &  0.995 & \textbf{0.999} \\
% 			\textbf{TA-Opt (L)} &
% 			\multicolumn{1}{c}{--} &  \textbf{0.045} & \textbf{0.156} &  \textbf{2.275} & \textbf{0.073} &  \textbf{0.978} &  \textbf{0.996} & \textbf{0.999} \\
% 			\midrule
			
% 			\textit{Improvement} & \textit{v.s. previous-best} &
% 			\textcolor{blue}{13.5$\%$} $\uparrow$  &
% 			\textcolor{blue}{17.9$\%$} $\uparrow$  &  \textcolor{blue}{3.6$\%$} $\uparrow$  &  \textcolor{blue}{17.0$\%$} $\uparrow$  &    \textcolor{blue}{14.5$\%$} $\uparrow$  & 
% 			\textcolor{blue}{0.1$\%$} $\uparrow$  &  \multicolumn{1}{c}{--} \\
% 			% 		\textit{Improvement} & \textit{v.s. previous-best} &
% 			% 		\textcolor{blue}{19.0$\%$} $\uparrow$  &
% 			% 		\textcolor{blue}{8.4$\%$} $\uparrow$  &  \textcolor{blue}{0.3$\%$} $\uparrow$  &  \textcolor{blue}{12.5$\%$} $\uparrow$  &    \textcolor{blue}{1.0$\%$} $\uparrow$  &  \multicolumn{1}{c}{--} &  \multicolumn{1}{c}{--} \\
% 			\bottomrule
% 		\end{tabular}%
% 			}
% % 		\vspace*{-5mm}
% \end{table*}

\begin{table*}[t]
    \centering
	\footnotesize
	\setlength{\tabcolsep}{3.5pt}
	% For LaTeX tables use
% 	\vspace{-0.5em}
	\centering
	\resizebox{\textwidth}{!}
	{%
		\begin{tabular}{lcccccccccc}
			\toprule
			Method & Reference & Input & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$ & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ & FPS $\uparrow$\\  
			\midrule
			Xu et al. \cite{xu2018structured} & CVPR 2018 & Single-Frame & 0.122 & 0.897 & 4.677 & \multicolumn{1}{c}{--} &  0.818 &  0.954 & 0.985 & \multicolumn{1}{c}{--} \\
			DORN \cite{fu2018deep} & CVPR 2018 & Single-Frame & 0.072 & 0.307 & 2.727 & 0.120 & 0.932 & 0.984 & 0.995 & \multicolumn{1}{c}{--} \\
			Yin et al. \cite{yin2019enforcing} & ICCV 2019 & Single-Frame & 0.072 & \multicolumn{1}{c}{--} &  3.258 &  0.117 &  0.938 &  0.990 & 0.998 & \multicolumn{1}{c}{--} \\
			PackNet-SAN \cite{guizilini2021sparse} & CVPR 2021 & Single-Frame & 0.062 & \multicolumn{1}{c}{--} &  2.888 &  \multicolumn{1}{c}{--} &  0.955 &  \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} \\
			DPT* \cite{ranftl2021vision} & ICCV 2021 & Single-Frame & 0.062 & \multicolumn{1}{c}{--} &  2.573 &  0.092 &  0.959 &
			0.995 & 0.999 & \multicolumn{1}{c}{--} \\
			PWA \cite{lee2021patch} & AAAI 2021 & Single-Frame & 0.060 & 0.221 &  2.604 &  0.093 &  0.958 &  0.994 & 0.999 & \multicolumn{1}{c}{--} \\
			AdaBins \cite{bhat2021adabins} & CVPR 2021 & Single-Frame & 0.058 & 0.190 &  2.360 &  0.088 & 0.964 & 0.995 & 0.999 & 2.96 \\
			NeWCRFs \cite{yuan2022newcrfs} & CVPR 2022 & Single-Frame & \textbf{0.052} & \textbf{0.155} &  \textbf{2.129} &  \textbf{0.079} &  \textbf{0.974} &  \textbf{0.997} & \textbf{0.999} & \textbf{3.48} \\
			P3Depth \cite{patil2022p3depth} & CVPR 2022 & Single-Frame & 0.071 & 0.270 &  2.842 &  0.103 &  0.953 &  0.993 & 0.998 & \multicolumn{1}{c}{--} \\
% 			\midrule
% 			PackNet-SfM \cite{guizilini20203d}       & CVPR 2020    & M$\to${O} & 0.064 & 0.300  & 3.089 & 0.108 & 0.943 & 0.989   & 0.997 & \multicolumn{1}{c}{--} \\
			\midrule
			BANet \cite{tang2018ba}   & ICLR 2019  & Multi-Frame & 0.083 & \multicolumn{1}{c}{--} & 3.640 & 0.134 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}\\
% 			BA-Net9.51
			DeepV2D \cite{teed2019deepv2d}   & ICLR 2020  & Multi-Frame & 0.064& 0.350& 2.946& 0.120& 0.946& 0.982& 0.991 & 0.67 \\
            MaGNet \cite{bae2022multi} & CVPR 2022 & Multi-Frame & 0.054 & 0.162 & \textbf{2.158} &  0.083 &  0.971 &  \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} \\
            DRO \cite{gu2023dro} & RA-L 2023 & Multi-Frame & 0.059 & 0.230 &  2.799 &  0.092 &  0.964 &  0.994 & 0.998 & \textbf{6.25} \\
            % MonoRec & \multicolumn{1}{c}{--} & Multi-Frame & 0.050 & 0.295 &  2.266 &  0.082 &  0.973 &  0.991 & 0.9986 & \multicolumn{1}{c}{--} \\
         \textbf{CTA-Depth} & \multicolumn{1}{c}{--} & Multi-Frame &  \textbf{0.045} & \textbf{0.156} &  2.275 & \textbf{0.073} &  \textbf{0.978} &  \textbf{0.997} & \textbf{0.999} & 5.53\\
			% \textbf{CTA-Depth (L)} &
			% \multicolumn{1}{c}{--} & Multi-Frame & \textbf{0.045} & \textcolor{blue}{0.156} &  \textcolor{blue}{2.275} & \textbf{0.073} &  \textbf{0.978} &  \textcolor{blue}{0.996} & \textbf{0.999} & 3.70 \\
   %              \midrule
			% \textit{Improvement v.s. Previous Multi-Frame Best} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} &
			% \textcolor{blue}{13.0$\%$} $\uparrow$  &
			% \textcolor{blue}{3.7$\%$} $\uparrow$  &  \textcolor{blue}{5.4$\%$} $\downarrow$  &  \textcolor{blue}{12.0$\%$} $\uparrow$  &    \textcolor{blue}{0.7$\%$} $\uparrow$  & 
			% \textcolor{blue}{0.3$\%$} $\uparrow$  &  \textcolor{blue}{0.1$\%$} $\uparrow$ & \multicolumn{1}{c}{--}\\    
			% % \midrule
			% % \textit{Improvement v.s. Previous Multi-Frame Baseline} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} &
			% % \textcolor{blue}{20.3$\%$} $\uparrow$  &
			% % \textcolor{blue}{32.2$\%$} $\uparrow$  &  \textcolor{blue}{18.7$\%$} $\uparrow$  &  \textcolor{blue}{20.7$\%$} $\uparrow$  &    \textcolor{blue}{1.5$\%$} $\uparrow$  & 
			% % \textcolor{blue}{0.2$\%$} $\uparrow$  &  \textcolor{blue}{0.1$\%$} $\uparrow$ & \multicolumn{1}{c}{--}\\
			% \midrule
			% \textit{Improvement v.s. Previous Single-Frame Best} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} &
			% \textcolor{blue}{9.6$\%$} $\uparrow$  &
			% \textcolor{blue}{0.6$\%$} $\downarrow$  &  \textcolor{blue}{6.9$\%$} $\downarrow$ & \textcolor{blue}{7.6$\%$} $\uparrow$  &    \textcolor{blue}{0.4$\%$} $\uparrow$  & \multicolumn{1}{c}{--}  &  \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}\\
			% 		\textit{Improvement} & \textit{v.s. previous-best} &
			% 		\textcolor{blue}{19.0$\%$} $\uparrow$  &
			% 		\textcolor{blue}{8.4$\%$} $\uparrow$  &  \textcolor{blue}{0.3$\%$} $\uparrow$  &  \textcolor{blue}{12.5$\%$} $\uparrow$  &    \textcolor{blue}{1.0$\%$} $\uparrow$  &  \multicolumn{1}{c}{--} &  \multicolumn{1}{c}{--} \\
			\bottomrule		
% 		\begin{tabular}{lcccccccccc}
% 			\toprule
% 			Method, Publication Venues    & Input & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$ & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ & FPS $\uparrow$\\  
% 			\midrule
% 			Xu et al., CVPR18 \cite{xu2018structured} & Single-Frame & 0.122 & 0.897 & 4.677 & \multicolumn{1}{c}{--} &  0.818 &  0.954 & 0.985 & 6.25 \\
% 			DORN, CVPR18 \cite{fu2018deep} & Single-Frame & 0.072 & 0.307 & 2.727 & 0.120 & 0.932 & 0.984 & 0.995 & 6.25\\
% 			Yin et al., ICCV19 \cite{yin2019enforcing} & Single-Frame & 0.072 & \multicolumn{1}{c}{--} &  3.258 &  0.117 &  0.938 &  0.990 & 0.998 & 6.25\\
% 			PackNet-SAN, CVPR21 \cite{guizilini2021sparse} & Single-Frame & 0.062 & \multicolumn{1}{c}{--} &  2.888 &  \multicolumn{1}{c}{--} &  0.955 &  \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & 6.25\\
% 			DPT*, ICCV21\cite{ranftl2021vision} & Single-Frame & 0.062 & \multicolumn{1}{c}{--} &  2.573 &  0.092 &  0.959 &
% 			0.995 & \textcolor{blue}{0.999} & 6.25\\
% 			PWA\cite{lee2021patch} & AAAI 2021 & Single-Frame & 0.060 & 0.221 &  2.604 &  0.093 &  0.958 &  0.994 & \textcolor{blue}{0.999} & 6.25\\
% 			AdaBins\cite{bhat2021adabins} & CVPR 2021 & Single-Frame & 0.058 & 0.190 &  2.360 &  0.088 & 0.964 & 0.995 & \textcolor{blue}{0.999} & 6.25\\
% 			NeWCRFs\cite{patil2022p3depth} & CVPR 2022 & Single-Frame & \textcolor{blue}{0.052} & \textbf{0.155} &  \textbf{2.129} &  \textbf{0.079} &  \textcolor{blue}{0.974} &  \textbf{0.997} & \textcolor{blue}{0.999} & 6.25\\
% 			P3Depth, CVPR22 \cite{patil2022p3depth} & Single-Frame & 0.071 & 0.270 &  2.842 &  0.103 &  0.953 &  0.993 & 0.998  & 6.25\\
% 			PackNet-SfM, CVPR20 \cite{guizilini20203d}    & M$\to${O} & 6.25 & 0.064 & 0.300  & 3.089 & 0.108 & 0.943 & 0.989   & 0.997   \\
% 			BANet, CVPR20 \cite{tang2018ba} & Multi-Frame & 6.25  & 0.083 & \multicolumn{1}{c}{--} & 3.640 & 0.134 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}  \\
% 			DeepV2D, ICLR20 \cite{teed2019deepv2d}        & Multi-Frame & 6.25  & 0.064& 0.350& 2.946& 0.120& 0.946& 0.982& 0.991         \\
% 			DRO, - \cite{patil2022p3depth} & Multi-Frame & 6.25  & 0.059 & 0.230 &  2.799 &  0.092 &  0.964 &  0.994 & 0.998\\
% 			CTA-Depth & Multi-Frame & 6.25  &  0.047 & 0.174 &  2.352 & 0.077 &  0.974 &  0.995 & \textbf{0.999} \\
% 			\textbf{CTA-Depth (L)} & Multi-Frame & 6.25  & \textbf{0.045} & \textcolor{blue}{0.156} &  \textcolor{blue}{2.275} & \textbf{0.073} &  \textbf{0.978} &  \textcolor{blue}{0.996} & \textbf{0.999} \\
% 			\midrule
% 			\textit{Improvement v.s. Previous Multi-Frame Best} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} &
% 			\textcolor{blue}{23.7$\%$} $\uparrow$  &
% 			\textcolor{blue}{32.2$\%$} $\uparrow$  &  \textcolor{blue}{18.7$\%$} $\uparrow$  &  \textcolor{blue}{20.7$\%$} $\uparrow$  &    \textcolor{blue}{1.5$\%$} $\uparrow$  & 
% 			\textcolor{blue}{0.2$\%$} $\uparrow$  &  \textcolor{blue}{0.1$\%$} $\uparrow$ \\
% 			\midrule
% 			\textit{Improvement v.s. Previous Single-Frame Best} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} &
% 			\textcolor{blue}{13.5$\%$} $\uparrow$  &
% 			\textcolor{blue}{0.6$\%$} $\downarrow$  &  \textcolor{blue}{6.9$\%$} $\downarrow$ & \textcolor{blue}{7.6$\%$} $\uparrow$  &    \textcolor{blue}{0.4$\%$} $\uparrow$  & \textcolor{blue}{0.1$\%$} $\downarrow$  &  \multicolumn{1}{c}{--} \\
% 			% 		\textit{Improvement} & \textit{v.s. previous-best} &
% 			% 		\textcolor{blue}{19.0$\%$} $\uparrow$  &
% 			% 		\textcolor{blue}{8.4$\%$} $\uparrow$  &  \textcolor{blue}{0.3$\%$} $\uparrow$  &  \textcolor{blue}{12.5$\%$} $\uparrow$  &    \textcolor{blue}{1.0$\%$} $\uparrow$  &  \multicolumn{1}{c}{--} &  \multicolumn{1}{c}{--} \\
% 			\bottomrule
		\end{tabular}%
	}
 \caption{Quantitative results on KITTI Eigen split with the cap of 0-80m. 
 Note that the seven widely-used metrics are calculated  strictly following AdaBins  \protect\cite{bhat2021adabins}. 
 ``Abs Rel" error occupies the main ranking metric. 
% ``FPS" of some recent methods is calculated on the same Nvidia RTX A6000 GPU. 
 ``*" means using additional data for training. 
 We utilize bold to highlight the best results of single-frame methods and multi-frame methods.
 }
\label{table_kitti_2}       % Give a unique label
\vspace{-4mm}
\end{table*}
% Highlighting: , and color the second-best or previous-best and our performance gain over them in blue. \textbf{best}, \textcolor{blue}{previous-best or the second-best},   \textcolor{blue}{our improvement over the previous-best}
% \begin{table*}[t]
%     \centering
% 	\footnotesize
% 	\setlength{\tabcolsep}{3.5pt}
% 	% For LaTeX tables use
% % 	\vspace{-0.5em}
% 	\centering
% 	\resizebox{\textwidth}{!}
% 	{%
% 		\begin{tabular}{lcccccccccc}

% 		\end{tabular}%
% 			}
% We conducted an extensive experiments of monocular depth estimation on the commSinglest KITTI benchmark and two other popular datasets. In the following, we first briefly describe the datasets and the corresponding evaluation, and then present quantitative comparisons with the state-of-the-art in monocular depth estimation. 
%In the following, we first briefly describe the datasets and the corresponding evaluation and then present quantitative comparisons with the state-of-the-art in monocular depth estimation on three popular datasets.

% \begin{figure*}[ht]
% 	\centering
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000021_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000095_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000113_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000140_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000153_1.png}}
% 		\vspace{0.8pt}	
% 		\begin{footnotesize}
% 			\centerline{(a) Input images}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000021_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000095_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000113_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000140_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000153_1.png}}
% 		\vspace{0.8pt}	
% 		\begin{footnotesize}
% 			\centerline{(b) Results of DRO}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000021_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000095_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000113_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000140_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000153_1.png}}
% 		\vspace{0.8pt}
% 		\begin{footnotesize}
% 			\centerline{(c) Ours}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\caption{Qualitative comparisons given input images (a) from KITTI. Clearly, our method (c) yields more accurate depth maps compared to DRO (b); see particularly the regions marked by green boxes.}
% 	%Green rectangles indicate the important regions for result analysis. }
% 	%\vspace*{-2mm}
% 	\label{fig005}
% \end{figure*}
% \begin{figure*}[t]
% 	\centering
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000010.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000012.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000016.png}}
% 		\vspace{0.8pt}
	
% 		\begin{footnotesize}
% 			\centerline{(a) Input images}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000010_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000012_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000016_1.png}}
% 		\vspace{0.8pt}

% 		\begin{footnotesize}
% 			\centerline{(b) Our Results}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000010_2.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000012_2.png}}
% 		\vspace{0.8pt}

% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000016_2.png}}
% 		\vspace{0.8pt}
% 		\begin{footnotesize}
% 			\centerline{(c) Error Maps}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\caption{Qualitative results and error maps given input images from KITTI dataset. According to error maps (correct estimates are in blue and wrong estimates are in red color tSingles), our method yields accurate depth maps. }
% 	%Green rectangles indicate the important regions for result analysis. }
% % 	\vspace{-0.5em}
% 	\label{fig_demo002}
% \end{figure*}
\subsection{Datasets}
We evaluate our method on three public benchmark datasets, including KITTI, Virtual KITTI 2, and nuScenes. These datasets provide a large number of monocular temporal neighboring images in dynamic environments.
%Below, we shall briefly introduce each one of them.
% \vspace{-2mm}
%, including KITTI, Virtual KITTI 2, and nuScenesand the preferred training dataset both in the supervised and self-supervised monocular depth estimation. It contains over 93 thousand depth maps with corresponding raw LiDAR scans and RGB images, aligned with the raw data. Our work performs monocular depth estimation on the widely used KITTI Eigen split \cite{eigen2014depth}. This split is composed of 22,600 images from 32 scenes for training and 697 images from 29 scenes for testing with LiDAR-based ground truth. The corresponding depth of each RGB image is sampled sparsely by the rotating LiDAR sensor.

\noindent\textbf{KITTI} \cite{geiger2012we} is a popular benchmark for the task of autonomous driving, which provides over 93,000 depth maps with corresponding raw LiDAR scans and RGB images aligned with raw data. In experiments, we follow the widely-used KITTI Eigen split \cite{eigen2014depth} for network training, which is composed of 22,600 images from 32 scenes for training and 697 images from 29 scenes for testing. The corresponding depth of each RGB image is sampled sparsely by the LiDAR sensor.

\noindent\textbf{Virtual KITTI 2} \cite{gaidon2016virtual} is widely used for video understanding tasks, which consists of 5 sequence clones from the KITTI tracking benchmark and contains 50 high-resolution monocular videos generated from five different virtual worlds in urban settings under various imaging and weather conditions. These photo-realistic synthetic videos are fully annotated with depth labels.

\noindent\textbf{nuScenes}~\cite{caesar2020nuscenes} is a large-scale multi-modal autonomous driving dataset that is the first to carry the completely autonomous vehicle sensor suite: 32-beam LiDAR, 6 cameras and 5 radars with 360° coverage. It comprises 1,000 scenes, where each scene lasts 20 seconds and is fully annotated with 3D bounding boxes for 23 classes and 8 attributes.

\subsection{Implementation Details}
We implement our CTA-Depth in PyTorch and train it for 100 epochs with a mini-batch size of 4. 
The learning rate is $2\times10^{- 4}$ for both depth and pose refinement, which is decayed by a constant step (gamma=$0.5$ and step size=$30$). 
We set $\beta_1=0.9$ and $\beta_2=0.999$ in the Adam optimizer. 
We resize the input images to $320\times960$ for training, and set the number of sequential images to 2 for CTA-Refiner by balancing both computation efficiency and prediction accuracy. For long-range geometry embedding, the number of temporally adjacent images is set to $N=3$. Since the output $\varphi(F_j)$ of the LGE for the same image is fixed and not updated with the iterations, this provides more prior temporal information to CTA-Refiner while ensuring network efficiency.
% \textcolor{red}{ADD NUMBER OF FRAMES USED FOR EMBEDDING}.
We fix $m$ at 3 and $n$ at 4 in experiments.

% set the number to 2, not set the number to be 2
% As described in Section \nameref{subsec:embed}, we have two solutions: CTA-Depth and CTA-Depth (L).
%We trained our network on four Nvidia RTX A6000 GPUs. 
%Generally speaking, it takes about two days for training on KITTI dataset.
% Generally speaking, it takes about two days for training and \xz{$XX$} hours for inference on KITTI dataset.

%deployed it on \xz{XX} Nvidia RTX A6000 GPUs. The network is trained for 200 epochs with a batch size of 4. For the optimizer, we employ Adam and set $\beta_{\text{1}}$ to 0.9 and $\beta_\text{2}$ to 0.999. The learning rate is set to 0.0002 for both depth and pose head and is decayed by constant step (gamma = 0.5, step size = 30). The input image is resized as 320 * 960. We use the loss functions and two-view setting proposed by previous excellent work \cite{gu2023dro} to optimize the TransOpt network. The training losses for supervised and self-supervised schemes are used for our monocular depth estimation tasks. In detail, the $\gamma$ is set to 0.85 in supervised training. The $\alpha$ is set to 0.85 and the $\lambda$ is set to 0.01 in self-supervised training.
\begin{figure*}[ht]
	\centering
	\begin{minipage}{0.32\linewidth}
		%\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000021_1.png}}
		%\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000095_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000113_1.png}}
        \centerline{\includegraphics[width=\textwidth]{Images/F5/F5_input_3.pdf}}
		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000140_1.png}}
% 		\vspace{0.8pt}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_input_2.pdf}}
		\vspace{0.8pt}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_input_1.pdf}}
		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_1/0000000153_1.png}}
% 		\vspace{0.8pt}	
		\begin{footnotesize}
			\centerline{(a) Input images}
		\end{footnotesize}
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
		%\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000021_1.png}}
		%\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000095_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000113_1.png}}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_dro_33.pdf}}
		\vspace{0.8pt}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_dro_22.pdf}}
		\vspace{0.8pt}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_dro_1.pdf}}
		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_2/0000000153_1.png}}
% 		\vspace{0.8pt}	
		\begin{footnotesize}
			\centerline{(b) Results of the Baseline}
		\end{footnotesize}
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
		%\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000021_1.png}}
		%\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000095_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000113_1.png}}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_our_3.pdf}}
		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000140_1.png}}
% 		\vspace{0.8pt}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_our_2.pdf}}
		\vspace{0.8pt}
		\centerline{\includegraphics[width=\textwidth]{Images/F5/F5_our_1.pdf}}
		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_img_3/0000000153_1.png}}
% 		\vspace{0.8pt}
		\begin{footnotesize}
			\centerline{(c) CTA-Depth (Ours)}
		\end{footnotesize}
	\end{minipage}
	\caption{Qualitative comparisons given input images (a) from KITTI. Clearly, our method (c) yields more accurate depth maps than the Baseline method; (b) see particularly the regions marked by green boxes.}
	%Green rectangles indicate the important regions for result analysis. }
	\vspace*{-2mm}
	\label{fig005}
\end{figure*}
% \begin{table*}[t]
% 	\footnotesize
% 	\setlength{\tabcolsep}{3.5pt}
% 	% table caption is above the table
% 	\caption{Ablation study on the KITTI dataset. 
% 		GRU: GRU module. Alter: alternate update. TransOpt: our TransOptimizer module. Cost: cost map. Highlighting: \textcolor{blue}{TA-Opt}, \textbf{TA-Opt (L)}. }
% % 	\vspace{-0.5em}
% 	\label{tableAblationStudy}       % Give a unique label
% 	% For LaTeX tables use
% 	\centering
% 	\begin{tabular}{lcccccc}
% 		\toprule
% 		Methods & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$ & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ \\
% 		\midrule\
% % 		w/o Cost & 0.061 & 0.305 & 3.183 & 0.109  & 0.942 & 0.989 \\
% % 		w/o GRU &  0.056 & 0.239 &  2.835 &  0.093 &  0.956 &  0.992 \\ 
% % 		w/o Alter & 0.053 & 0.224 & 2.823 & 0.091 & 0.963 & 0.992 \\
% % 		w/o TransOpt & 0.047 & 0.199 & 2.629 & 0.082 & 0.970 & 0.994 \\ 
% 		DRO & 0.047 & 0.199 & 2.629 & 0.082 & 0.970 & 0.994 \\
% 		\textcolor{blue}{TA-Opt} (Res-18) & \textcolor{blue}{0.040} & \textcolor{blue}{0.157} & \textcolor{blue}{2.288} & \textcolor{blue}{0.071} & \textcolor{blue}{0.977} & \textcolor{blue}{0.996} \\
% 		\textbf{TA-Opt (L)} (Swin-L) & \textbf{0.037} & \textbf{0.139} & \textbf{2.191} & \textbf{0.068} & \textbf{0.980} & \textbf{0.996} \\ 
% 		\bottomrule
% 	\end{tabular}

% % DRO\cite{gu2023dro}               & Multi             &\multicolumn{1}{c}{\Checkmark}            &Improved& \textcolor{blue} {0.047}& \textcolor{blue} {0.199}& 2.629& \textcolor{blue} {0.082}& \textcolor{blue} {0.970}& 0.994& 0.998
%\vspace*{-2mm}
% \end{table*}
\subsection{Computation Time Analysis}
Given the same Nvidia RTX A6000 GPU on the KITTI dataset, compared to the state-of-the-art one-frame method NeWCRFs \cite{yuan2022newcrfs}, the inference speed of our CTA-Depth, i.e., the number of images inferred per second (FPS), is greatly improved by 58.9$\%$, i.e., 5.53 (Ours) vs. 3.48 (NeWCRFs). This is because NeWCRFs use four swin-large transformers as multi-level encoders, while our method uses the lightweight ResNet18 backbone as the encoder to extract features. 
On the other hand, as shown in Table \ref{table_kitti_2}, although the FPS of CTA-Depth is slightly lower than that of the multi-frame method DRO \cite{gu2023dro} (5.53 vs. 6.25),  our performance significantly outperforms DRO and MaGNet \cite{bae2022multi}.


%at the pixel level with category, instance, flow, and depth labels. 
%to better learn and evaluate computer vision models for several video understanding tasks including depth estimation and object detection.
% \begin{table*}[t]
% 	\footnotesize
% 	\setlength{\tabcolsep}{3.5pt}
% 	% table caption is above the table
% 	\caption{Quantitative results on a subset of the Virtual KITTI 2. Highlighting: \textbf{best}, \textcolor{blue}{our improvement}. }
% % 	\vspace{-0.5em}
% 	\label{table_vkitti01}       % Give a unique label
% 	% For LaTeX tables use
% 	\centering
% 	\begin{tabular}{lcccccc}
% 		\toprule
% 		Method             & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$ & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ \\
% 		\midrule
% 		GLPDepth & 0.058 & 0.217 &  2.146 &  0.125 &  0.928 &  0.987 \\
% 		Adabins & 0.041 & 0.164 & 1.981 & 0.094 &  0.962 & 0.990\\
% 		DRO & 0.040 & 0.153 &  1.903 &  0.092 &  0.967 &  0.990 \\ 
% 		\textbf{TA-Opt (Ours)}  & \textbf{0.035} & \textbf{0.129} &  \textbf{1.715} &  \textbf{0.085} &  \textbf{0.976} &  \textbf{0.993} \\
% 		\midrule
		
% 		\textit{Improvement} & \textcolor{blue}{12.5$\%$} $\uparrow$ & \textcolor{blue}{15.7$\%$} $\uparrow$ &  \textcolor{blue}{9.9$\%$} $\uparrow$ &  \textcolor{blue}{7.6$\%$} $\uparrow$ &  \textcolor{blue}{0.9$\%$} $\uparrow$ & \textcolor{blue}{0.3$\%$} $\uparrow$ \\
% 		\bottomrule
% 	\end{tabular}
% 	%\vspace*{-2mm}
% \end{table*}

% \begin{table*}[t]
% 	\footnotesize
% 	\setlength{\tabcolsep}{3.5pt}
% 	% table caption is above the table
% 	\caption{Quantitative results on a subset of the nuScenes dataset. Highlighting: \textbf{best}, \textcolor{blue}{our improvement}. }
% % 	\vspace{-0.5em}
% 	\label{table_nus01}       % Give a unique label
% 	% For LaTeX tables use
% 	\centering
% 	\begin{tabular}{lcccccc}
% 		\toprule
% 		Method             & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$ & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ \\
% 		\midrule
% 		GLPDepth & 0.061 & 0.340 & 3.159 &  0.121 &  0.925 &  0.984 \\
% 		Adabins & 0.058 & 0.314 & 3.156 & 0.117 &  0.940 &  0.985 \\	DRO &  0.057 & 0.303 &  3.004 &  0.114 &  0.942 &  0.985 \\
% 		\textbf{CTA-Depth (Ours)}  &  \textbf{0.050} & \textbf{0.252} &  \textbf{2.786} &  \textbf{0.104} &  \textbf{0.962} &  \textbf{0.988} \\
% 		\midrule
% 		\textit{Improvement} & \textcolor{blue}{12.3$\%$} $\uparrow$ & \textcolor{blue}{16.8$\%$} $\uparrow$ &  \textcolor{blue}{7.3$\%$} $\uparrow$ &  \textcolor{blue}{8.8$\%$} $\uparrow$ &  \textcolor{blue}{2.1$\%$} $\uparrow$ & \textcolor{blue}{0.3$\%$} $\uparrow$ \\
% 		\bottomrule
% 	\end{tabular}
% \vspace*{-2mm}
% \end{table*}


\subsection{Evaluation of Our Method}
% \subsection{Comparison with State-of-the-Arts}

\paragraph{Evaluation on KITTI.} 
We first compare our CTA-Depth against top performers of supervised monocular depth estimation on the KITTI dataset; see Tables \ref{table_kitti_1} \& \ref{table_kitti_2} for the results. For a fair comparison, all methods are evaluated given the same sequential images. %Tables~\ref{table_kitti_1} \& \ref{table_kitti_2} summarize the quantitative comparison results.
In Table \ref{table_kitti_1}, the seven widely-used evaluation metrics are calculated strictly following the work~\cite{gu2023dro} and the ground-truth median scaling is applied to obtain the final output.
% In contrast, the seven evaluation metrics in Table~\ref{table_kitti_2} are calculated according to AdaBins~\cite{bhat2021adabins} and the final output is calculated by taking the average prediction of the image and its mirror image. We also evaluate our method against others in terms of the reference speed (FPS) using the same Nvidia RTX A6000 GPU. Clearly, both CTA-Depth and CTA-Depth (L) achieve the state-of-the-art performance over all the evaluation metrics under two different evaluation strategies with significant improvements. 
In contrast, the seven evaluation metrics in Table~\ref{table_kitti_2} are calculated according to AdaBins~\cite{bhat2021adabins} and the final output is calculated by taking the average prediction of the image and its mirror image. 
We also evaluate our method against others in terms of the reference speed (FPS) using the same Nvidia RTX A6000 GPU. Clearly, CTA-Depth achieves state-of-the-art performance over all the evaluation metrics under two different evaluation strategies.


% Note that, "M$\rightarrow$O" means monocular multiple frame images are used in training while only one image is used for inference.Clearly, as shown in both two tables, our method (including two versions CTA-Depth and CTA-Depth (L)) achieves the highest values over all the evaluation metrics under two different calculation strategies with significant improvements (see the bottom-most row).
% ; see these regions marked by green boxes
We further show the qualitative comparisons in Fig.~\ref{fig005} by comparing our method (c) with the recent approach \cite{gu2023dro} (b).
As shown in the green boxes, our method yields finer depth estimation results for moving objects in dynamic scenes, small objects and object contours, such as the trams and traffic signs. In addition, as shown in the top row of Fig.~\ref{fig005}, our predicted depth map for the tram window is more consistent with the rest parts of the tram. 
% \vspace{-2mm}
% Moreover, we also show the visual comparisons in Fig.~\ref{fig005} by comparing our method (c) with the recent baseline DRO (b).
% As shown in the green boxes, our method yields finer depth estimation results for moving objects, small objects and object contours, such as pedestrians and traffic signs. In addition, as shown in the second and third rows of Fig.~\ref{fig005}, our predicted depth maps generated by our method for the tram window are more consistent with the rest parts of the tram. 
% More visual results and error maps are shown in Fig.~\ref{fig_demo002}. In error maps, correct estimates are in blue and wrong estimates are in red. Clearly, our method yields accurate depth maps.

%We compare our TransOpt with top performers for monocular depth estimation under both self-supervised and supervised learning schemes. The self-supervised scheme use the setting and loss functions based on DRO\cite{gu2023dro}. For a fair comparison, all methods are evaluated under the two-view setting. The results show that our method leads to a decisive improvement in the state-of-the-art on KITTI benchmark. Results
%on two ground-truth types are displayed since different methods are evaluated using different types. ‘M$\rightarrow$O’ means multiple images are
%used in the training while one image is used for inference. The quantitative and qualitative results are shown in Table \ref{table_kitti_1} and Figure \ref{fig005} respectively. We can see that our method achieves finer depth estimation results for small objects and object contours, such as pedestrians, traffic signs, etc. Furthermore, the enhancement of global feature learning by our TransOpt module also enables our model to perform better on the depth consistency of objects. As can be seen in the second and third rows of Figure \ref{fig005}, the depth maps generated by our method for the tram window are more consistent with the rest parts of the tram.

%We use two different evaluation metrics to compare current top performers fairly. In Table \ref{table_kitti_1}, we employ the evaluation metrics used by the DRO\cite{gu2023dro} method and apply ground-truth median scaling to the final prediction output. In Table \ref{table_kitti_2}, without ground-truth median scaling, the final prediction output is calculated by taking the average of an image’s prediction and the prediction of its mirror image according to the AdaBins\cite{bhat2021adabins} method. According to Table \ref{table_kitti_2}, our method achieves state-of-the-art results compared to the transformer-based methods including AdaBins\cite{bhat2021adabins}, DPT-Hybrid\cite{ranftl2021vision}, and the well-known method BTS\cite{lee2019big}.
\paragraph{Evaluation on Virtual KITTI 2.} We further verify our method on the virtual KITTI 2 dataset as shown in Table \ref{table_vkitti01}. 
We use a subset of the virtual KITTI 2, which contains 1,700 images for training and 193 images for testing. 
%The performance of our method compared with the most relevant method DRO \cite{gu2023dro} is shown in Table \ref{table_vkitti01}.
Notably, our CTA-Depth achieved significantly better results than the multi-frame baseline methods over all evaluation metrics.
% Notably, our CTA-Depth has achieved significantly better results than the multi-frame baseline methods over all evaluation metrics, even without the full pipeline CTA-Depth (L).
% \vspace{-2mm}
\paragraph{Evaluation on nuScenes.} To further demonstrate the competitiveness of our approach, we also conduct an evaluation on the nuScenes dataset. 
%Similarly, only the supervised learning scheme is used.
In this experiment, we manually split a subset consisting of 2,600 images for training and 170 images for testing. The result is shown in Table \ref{table_nus01}. Again, the results show that our proposed method outperforms the baselines with a significant margin in all evaluation metrics.
% \vspace{-2mm}
\begin{table}[t]
	\footnotesize
	\setlength{\tabcolsep}{3.5pt}
    % 	\vspace{-0.5em}
	% For LaTeX tables use
	\centering
	\begin{tabular}{lcccc}
		\toprule
		Method & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$\\
		\midrule
		GLPDepth & 0.058 & 0.217 &  2.146 &  0.125 \\
		Adabins & 0.041 & 0.164 & 1.981 & 0.094 \\
		DRO & 0.040 & 0.153 &  1.903 &  0.092 \\ 
		\textbf{CTA-Depth}  & \textbf{0.035} & \textbf{0.129} &  \textbf{1.715} &  \textbf{0.085} \\
		\midrule
		% \textit{Improvement} & \textcolor{blue}{12.5$\%$} $\uparrow$ & \textcolor{blue}{15.7$\%$} $\uparrow$ &  \textcolor{blue}{9.9$\%$} $\uparrow$ &  \textcolor{blue}{7.6$\%$} $\uparrow$ \\
		\bottomrule
	\end{tabular}
	\caption{Quantitative results on a subset of the Virtual KITTI 2. }
 % Highlighting: \textbf{best}. , \textcolor{blue}{our improvement}
        \vspace{-3mm}
	\label{table_vkitti01}       % Give a unique label
\end{table}

\begin{table}[t]
	\footnotesize
	\setlength{\tabcolsep}{3.5pt}
    % 	\vspace{-0.5em}
	% For LaTeX tables use
	\centering
	\begin{tabular}{lcccc}
		\toprule
		Method             & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$\\
		\midrule
		GLPDepth & 0.061 & 0.340 & 3.159 &  0.121 \\
		Adabins & 0.058 & 0.314 & 3.156 & 0.117\\	DRO &  0.057 & 0.303 &  3.004 &  0.114 \\
		\textbf{CTA-Depth}  &  \textbf{0.050} & \textbf{0.252} &  \textbf{2.786} &  \textbf{0.104} \\
		% \midrule
		% \textit{Improvement} & \textcolor{blue}{12.3$\%$} $\uparrow$ & \textcolor{blue}{16.8$\%$} $\uparrow$ &  \textcolor{blue}{7.3$\%$} $\uparrow$ &  \textcolor{blue}{8.8$\%$} $\uparrow$ \\
		\bottomrule
	\end{tabular}
	\caption{Quantitative results on a subset of the nuScenes dataset. }
	\vspace{-3mm}
	\label{table_nus01}       % Give a unique label
\end{table}

\subsection{Ablation Study}

\begin{table}[t]
	\footnotesize
	\setlength{\tabcolsep}{3.5pt}
	% For LaTeX tables use
	\centering
	\begin{tabular}{lccccc}
		\toprule
	Setting & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$ $\downarrow$\\
% 	    \midrule
% 	w/o Cost & 0.065 & 0.324 & 3.270 & 0.112 & 0.940 & 0.988 \\
% 	Cost volume & 0.049 & 0.214 & 2.804 & 0.086 & 0.966 & 0.994 \\
% 	Baseline & 0.047 & 0.199 & 2.629 & 0.082 & 0.970 & 0.994 \\
% Baseline & 0.065 & 0.325 & 3.279 & 0.113 \\
%         + Refiner & 0.047 & 0.199 & 2.629 & 0.082 \\
%         + Depth-CTA & 0.044 & 0.178 & 2.463 & 0.077 \\
%         + Pose-CTA & 0.042 & 0.161 & 2.357 & 0.074 \\
% 	+ TEM & 0.040 & 0.157 & 2.288 & 0.071 \\
% 	+ M  & 0.040 & 0.155 & 2.276 & 0.071 \\
% 	+ M + C & 0.039 & 0.151 & 2.253 & 0.070 \\ 
% 	+ MAE  & 0.038 & 0.145 & 2.224 & 0.069 \\
	    \midrule
	Baseline & 0.060 & 0.275 & 3.132 & 0.104 \\
        + Multi-level & 0.059 & 0.267 & 3.105 & 0.101 \\
	+ Cross-scale & 0.057 & 0.248 & 2.951 & 0.096\\
	+ MAE  & 0.056 & 0.243 & 2.930 & 0.094 \\
        + Depth-CTA & 0.051 & 0.192 & 2.586 & 0.082 \\
        + Pose-CTA & 0.047 & 0.169 & 2.307 & 0.075 \\
	+ LGE & 0.045 & 0.156 & 2.275 & 0.073 \\
	
	% + M + E + R + P + S & 0.037 & 0.139 & 2.191 & 0.068 \\
 %        Baseline & 0.047 & 0.199 & 2.629 & 0.082 \\
	% CTA-Refiner & 0.040 & 0.157 & 2.288 & 0.071 \\
	% + M  & 0.040 & 0.155 & 2.276 & 0.071 \\
	% + M + C & 0.039 & 0.151 & 2.253 & 0.070 \\ 
	% + M + E + R & 0.039 & 0.148 & 2.245 & 0.070 \\
	% + M + E + R + P & 0.038 & 0.145 & 2.224 & 0.069 \\
	% + M + E + R + P + S & 0.037 & 0.139 & 2.191 & 0.068 \\
% 		\midrule\
% 	    16, 8, 4, 2 & 0.038 & 0.139 & 2.191 & 0.068 & 0.980 & 0.996 \\
% 		32, 16, 8, 4 & 0.037 & 0.139 & 2.191 & 0.068 & 0.980 & 0.996 \\
		\midrule
	$I_{t-1}$, $I_t$ & 0.050 & 0.221 & 2.813 & 0.089 \\
	$I_{t-2}$, $I_{t-1}$, $I_t$ & 0.048 & 0.215 & 2.807 & 0.086 \\
	$I_{t-1}$, $I_t$, $I_{t+1}$  & 0.045 & 0.156 & 2.275 & 0.073 \\
		\bottomrule
	\end{tabular}
	\caption{Ablation study on the KITTI dataset. "Multi-level" refers to multi-level feature extraction, "Cross-scale" refers to cross-scale attention layers, "CTA" refers to context-aware temporal attention. "$I_{t-i}$" is the input frame at time $t-i$.}
	\vspace*{-2mm}
	\label{tableAblationStudy}       % Give a unique label
\end{table}
%"Depth-CTA" and "Pose-CTA" refers to depth and pose context-aware temporal attention, respectively.Table \ref{tableAblationStudy} summarizes the ablation study results of each major module in our method on KITTI dataset.
To inspect the importance of each module in our method, we conduct an ablation study on the KITTI dataset and provide the results in Table \ref{tableAblationStudy}. From top to bottom, the proposed modules are added in turn until the full method is constructed.

\noindent\textbf{Baseline.} To verify the effectiveness of each component, we build a baseline model. 
This model has a similar network architecture as the full pipeline, which includes the encoder-decoder structure with a deep recurrent network. 
In other words, the proposed CTA module and LGM are removed.
The MAE module keeps only the single-level ResNet18 feature net for the depth and pose estimations.
% based on the baseline, we only replace its recurrent optimizer with our CTA-Refiner.and gain a significant performance improvement as shown in Table \ref{tableAblationStudy}. 
% Clearly, "Abs Rel" error is reduced from 0.047 to 0.040, demonstrating the effectiveness of the context-aware temporal attention based refinement network in depth estimation.

% we train our CTA-Depth model with the exactly same setting as the baseline DRO\cite{gu2023dro} model. In other words, 


% To verify the effectiveness of different components in multi-level attention enhanced predictor, we turn them on and off in turn as shown in Table \ref{tableAblationStudy}.

% \textbf{Multi-level feature extraction.} \lzz{Compared with baseline method, which only extract the feature maps with the 1/8 resolution of the input images, we extract four levels feature maps as shown in Fig.~\ref{fig:encoder}. The performance increment shows that multi-level features provide more valuable information.}

\noindent\textbf{Multi-level feature extraction.} We extract four levels of feature maps as shown in Fig.~\ref{fig:encoder}. The performance gain shows that it provides more valuable information for the model.

\noindent\textbf{Cross-scale attention.} Next, we use the same ResNet18 as the feature encoder and add cross-scale attention layers to decode the features at each level following Fig.~\ref{fig:encoder}.
%, which effectively maintains the global information interaction. 
% As shown in Table \ref{tableAblationStudy}, the cross-scale attention decoder leads to a performance increase.
%  Unlike DRO, the initial depth maps are obtained directly from the ResNet18 and a depth head, we use ResNet18 as the feature encoder and add cross-attention layers to decode the features at each level, which effectively maintains the global information interaction. 
% employ an encoder-decoder network to yield the initial predictions. the initial depth and pose predictions are obtained directly from the ResNet18 network and a depth head.In addition to the two operations above, the rearrange upscale is added to reduce the network complexity. Together with the PPM, they consequently enhance the estimation performance.

\noindent\textbf{MAE module.} In addition to the two operations above, the rearrange upscale is added to reduce the network complexity. Together with the PPM, they consequently enhance the estimation performance.
% \textbf{Swin-transformer encoder.} \lzz{In this step, we replace ResNet18 encoder with swin-transformer encoder and name this large network scheme as TA-Opt (L). For baseline and our TA-Opt, the main contribution is the optimization module. Since the optimization of depth and pose is a coarse-to-fine process, the initial predictions do not need to be very precise. Nevertheless, a stronger initial predictor still leads to an overall performance improvement of the framework.}

\noindent\textbf{Depth-CTA and Pose-CTA.} We add Depth-CTA and Pose-CTA after the cost map to obtain dynamic features by implicitly modeling the temporal relation and learn the geometric constraints through the temporal frames. In this way, the learned adaptive dynamic features are fed to the GRU optimizers and yield a noticeable performance gain. The "Abs Rel" error is reduced from 0.056 to 0.047. Furthermore, Fig.~\ref{fig:teaser} demonstrates the effectiveness of CTA modules in estimating accurate depths in dynamic environments.
%  Unlike DRO, the initial

\noindent\textbf{LGE.} The long-range geometry embedding module provides temporal priors for dynamic objects in several temporal neighboring frames and enhances the learning of the CTA module by large margins. 
% \noindent\textbf{Swin-transformer encoder.} In this step, we replace ResNet18 encoder with swin-transformer encoder and name this large network scheme as CTA-Depth (L), which also further improves the performance.

\noindent\textbf{Multi-frame input.} Here, we set up three experiments with different numbers of input frames. The results show that the optimal performance is achieved when the adopted temporal frames are $I_{t-1}$, $I_t$ and $I_{t+1}$, i.e., two image pairs: ($I_{t-1},I_{t}$) and ($I_{t},I_{t+1}$).
However, the network becomes over-complicated and time-consuming to train or infer when utilizing more than three sample frames for depth refinement.
% \lzz{which can be reasoning as this combination contains the most image information for the moving object of the current reference frame $I_t$.} 


% . of replacing baseline's lightweight ResNet18 encoder with a larger network in exchange 
% To verify the effectiveness of the proposed neural window fully-connected FC-CRFs, we build a baseline model. and obtain a noticeable performance improvement as shown in Table 5. The “Abs Rel” error is reduced from 0.069 to 0.055, and then to 0.054 by adding the shift action. This demonstrates the effectiveness of theneural window FC-CRFs in estimating accurate depths.


% Clearly, the feature-based cost map is a critical module, since the absolute relative error (Abs Rel) climbs from 0.037 (bottom row) to 0.061 (first row) without it. 
% Further, the GRU module is also important since it reduces the Abs Rel by 0.019. 
% Finally, even with installing the cost and GRU modules, our TA-Opt and TA-Opt (L) networks improve the quantitative results with a significant margin.

% \begin{table}
%   \caption{Sample table title}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}
% \vspace{-2mm}

% \lzz{This is because CTA-Depth uses the lightweight backbone ResNet18 as the feature encoder, compared to the large swin-transformer encoder of NeWCRFs.}
% \begin{figure*}[t]
% 	\centering
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000010.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000012.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000016.png}}
% 		\vspace{0.8pt}
	
% 		\begin{footnotesize}
% 			\centerline{(a) Input images}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000010_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000012_1.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000016_1.png}}
% 		\vspace{0.8pt}

% 		\begin{footnotesize}
% 			\centerline{(b) Our Results}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000010_2.png}}
% 		\vspace{0.8pt}
% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000012_2.png}}
% 		\vspace{0.8pt}

% 		\centerline{\includegraphics[width=\textwidth]{Images/demo_im01/0000000016_2.png}}
% 		\vspace{0.8pt}
% 		\begin{footnotesize}
% 			\centerline{(c) Error Maps}
% 		\end{footnotesize}
% 	\end{minipage}
% 	\caption{Qualitative results and error maps given input images from KITTI dataset. According to error maps (correct estimates are in blue and wrong estimates are in red color tones), our method yields accurate depth maps. }
% 	%Green rectangles indicate the important regions for result analysis. }
% % 	\vspace{-0.5em}
% 	\label{fig_demo002}
% \end{figure*}

% Compared with DRO, though the FPS of our method is slightly lower than DRO (\xz{XX} vs. \xz{XX}), our performance is significantly better than it.

%Our TA-Opt utilizes the lightweight network ResNet-18 as the backbone. We compare TA-Opt with our baseline DRO and previous state-of-the-art method Adabins in terms of the run-time and memory consumption, since TA-Opt has already outperformed others. The experiments are conducted on KITTI with an Nvidia RTX A6000 GPU. Compared to Adabins, our method achieves better depth accuracy while taking less inference time. The inference speed of our TA-Opt, i.e., the number of images inferred per second (FPS), is improved by 77.7$\%$ compared to Adabins on the same platform.

% \begin{table}
% 	\footnotesize
% 	\setlength{\tabcolsep}{2.8pt}
% 	% table caption is above the table
% 	\caption{Efficiency experiments on the KITTI dataset.}
% 	\vspace{-0.5em}
% 	\label{tableMemory}       % Give a unique label
% 	\centering
% 	\begin{tabular}{lcccc}
% 		\toprule
% 		Models & \begin{tabular}[c]{@{}c@{}}Resolution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory(G)\end{tabular} &
% 		\begin{tabular}[c]{@{}c@{}}Time(s)\end{tabular} &
% 		\begin{tabular}[c]{@{}c@{}}Abs Rel\end{tabular}  \\
% 		\midrule
% 		DeepV2D         & 192*1088   & 6.75      & ---    & 0.064 \\ 
% 		DRO(iterate 12) & 320 * 960  & 1.74     & 0.16    & 0.047 \\ 
% 		ours            & 320 * 960   & 2.74          & 0.19        & 0.044  \\
% 		\bottomrule
% 	\end{tabular}
% \end{table}



% \toprule
% 			Method            & Input  & Supervised            & GT type & Abs Rel $\downarrow$  & Sq Rel $\downarrow$ & RMSE $\downarrow$ & RMSE$_{log}$  $\downarrow$   & $\delta_1 < 1.25$ $\uparrow$ & $\delta_2 < 1.25^2$ $\uparrow$ & $\delta_3 < 1.25^3$ $\uparrow$ \\ \midrule
% % 			SfMLearner\cite{zhou2017sfm}        & M$\to${O}    &\multicolumn{1}{c}{\XSolidBrush}            &Velodyne& 0.208& 1.768& 6.856& 0.283& 0.678& 0.885& 0.957         \\
% % 			CCNet\cite{ranjan2019cc}             & M$\to${O}    &\multicolumn{1}{c}{\XSolidBrush}            &Velodyne& 0.140& 1.070& 5.326& 0.217& 0.826& 0.941& 0.975         \\
% % 			GLNet\cite{chen2019glnet}             & M$\to${O}    &\multicolumn{1}{c}{\XSolidBrush}            &Velodyne& 0.135& 1.070& 5.230& 0.210& 0.841& 0.948& 0.980         \\
% % 			MonoDepth\cite{Godard2019monodepth}         & M$\to${O}    &\multicolumn{1}{c}{\XSolidBrush}            &Velodyne& 0.115& 0.882& 4.701& 0.190& 0.879& {0.961}& {0.982}         \\
% % 			PackNet-SfM\cite{guizilini20203d}       & M$\to${O}    &\multicolumn{1}{c}{\XSolidBrush}            &Velodyne& 0.107& 0.803& 4.566& 0.197& 0.876& 0.957& 0.979         \\
% % 			DRO\cite{gu2023dro}               & Multi              &\multicolumn{1}{c}{\XSolidBrush}            &Velodyne& 0.088& 0.797& 4.464& 0.212& 0.899& 0.959& 0.980         \\
% % 			TA-Opt (ours)            &         Multi          &\multicolumn{1}{c}{\XSolidBrush}            &  Velodyne        &  {0.083}      &    {0.775}    &   {4.355}    &  {0.206} &  {0.901}     &     0.959    &    0.980     \\
% % 			\midrule
% 			PackNet-SfM\cite{guizilini20203d}       & M$\to${O}   &\multicolumn{1}{c}{\Checkmark}            &Velodyne& 0.090& 0.618& 4.220& 0.179& 0.893& 0.962& 0.983         \\
% 			DRO\cite{gu2023dro}               & Multi             &\multicolumn{1}{c}{\Checkmark}            &Velodyne& 0.073& 0.528& 3.888& 0.163& 0.924& 0.969& 0.984         \\
% 			TA-Opt (ours)            &         Multi          &\multicolumn{1}{c}{\Checkmark}            & Velodyne         &   0.071      &     0.496   &   3.598    &   0.143    &   0.931    &    0.975     &  0.989      \\
% 			\midrule
% % 			MonoDepth\cite{Godard2019monodepth}         & M$\to${O}   &\multicolumn{1}{c}{\XSolidBrush}          & Improved & 0.090 & 0.545  & 3.942 & 0.137 & 0.914 & 0.983   & 0.995   \\
% % 			PackNet-SfM\cite{guizilini20203d}       & M$\to${O}   &\multicolumn{1}{c}{\XSolidBrush}         & Improved & 0.071 & 0.359  & 3.153 & 0.109 & 0.944 & {0.990}   & {0.997}   \\
% % 			DRO\cite{gu2023dro}               & Multi             &\multicolumn{1}{c}{\XSolidBrush}          & Improved & 0.057 & 0.342  & 3.201 & 0.123 & 0.952 & 0.989   & 0.996   \\
% % 			TA-Opt (ours)            &         Multi          &\multicolumn{1}{c}{\XSolidBrush}  &   Improved       &   {0.055}    &  {0.321}      &   {3.156}    &    {0.118}    &   {0.955}    &   0.989      &    0.996     \\
% % 			\midrule
% 			BANet\cite{tang2018ba}  & Multi  & \multicolumn{1}{c}{\Checkmark} & Improved & 0.083 & \multicolumn{1}{c}{--} & 3.640 & 0.134 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--}  \\
% 			DeepV2D(2-view)\cite{teed2019deepv2d}   & Multi             &\multicolumn{1}{c}{\Checkmark}            &Improved& 0.064& 0.350& 2.946& 0.120& 0.946& 0.982& 0.991         \\
% 			PackNet-Sfm\cite{guizilini20203d}       & M$\to${O}         &\multicolumn{1}{c}{\Checkmark}            & Improved & 0.064 & 0.300  & 3.089 & 0.108 & 0.943 & 0.989   & 0.997   \\
% 			BTS\cite{lee2019big}              &  Multi   &\multicolumn{1}{c}{\Checkmark}            & Improved & 0.059 & 0.241  & 2.756 & 0.096 & 0.956 & 0.993   & 0.998   \\
% 			DRO\cite{gu2023dro}               & Multi             &\multicolumn{1}{c}{\Checkmark}            &Improved& \textcolor{blue} {0.047}& \textcolor{blue} {0.199}& 2.629& \textcolor{blue} {0.082}& \textcolor{blue} {0.970}& 0.994& 0.998        \\
% 			GLPDepth\cite{kim2022global}   & Multi             &\multicolumn{1}{c}{\Checkmark}            &Improved& 0.057& \multicolumn{1}{c}{--}& \textcolor{blue} {2.297}& 0.086& 0.967& \textcolor{blue} {0.996}& \textcolor{blue} {0.999}         \\
% 			TA-Opt (Ours)            &         Multi          &\multicolumn{1}{c}{\Checkmark}            &   Improved       & 0.040       &    0.157  &   2.288    &  0.071     &   0.977    &    \textbf{0.996}     & \textbf{0.999}      \\
% 			\textbf{TA-Opt (L) (Ours)}            &         Multi          &\multicolumn{1}{c}{\Checkmark}            &   Improved       &  \textbf{0.037}       &     \textbf{0.139}   &   \textbf{2.191}    &  \textbf{0.068}     &   \textbf{0.980}    &    \textbf{0.996}     &   \textbf{0.999}      \\
% 			\midrule
% 			% ResNet-18 + TransOpt,Swin-L + TransOpt	
% 			\textit{Improvement}   & \multicolumn{1}{c}{--} & \textit{v.s. previous-best} & \multicolumn{1}{c}{--} & \textcolor{blue}{21.3$\%$} $\uparrow$ &  \textcolor{blue} {30.2$\%$} $\uparrow$ &  \textcolor{blue}{4.6$\%$} $\uparrow$ &  \textcolor{blue}{17.1$\%$} $\uparrow$ &  \textcolor{blue}{1.0$\%$} $\uparrow$ &  \multicolumn{1}{c}{--}& \multicolumn{1}{c}{--}\\ 
% 			\bottomrule
% 		\end{tabular}%
% 	}

==> introduction.tex <==
\section{Introduction}
% \new{Monocular depth estimation is the task of predicting an accurate depth value (distance relative to the camera) of each pixel from RGB images captured by a monocular camera.
% Due to its relatively low cost, small sensor size, and rich content of acquired information, monocular depth estimation has promising prospects for practical applications, 
% e.g., autonomous driving~\cite{li2022densely,9922174}, robot navigation~\cite{mumuni2022bayesian}, to name a few. Given the fact that temporal and spatially continuous images are available in most real-world scenarios, multi-frame monocular depth estimation methods~\cite{wang2019recurrent,zhang2019exploiting,patil2020don} are proposed to utilize the temporally neighboring frames and explore recurrent networks to improve the depth prediction accuracy.

Monocular depth estimation aims at predicting accurate pixel-wise depth from monocular RGB images.
Due to its low cost and easy implementation, monocular depth estimation has achieved promising prospects in practical applications~\cite{li2022densely,9922174,mumuni2022bayesian}.
Particularly, monocular depth estimation~\cite{li2015depth,liu2015deep,ricci2018monocular,bhat2021adabins,yuan2022newcrfs} under the single-frame setting has achieved convincing results by conducting robust convolutional neural networks with prior geometric constraints.
Nevertheless, it is still challenging to precisely recover the 3D environment from a single monocular 2D image. 
On the other hand, noting that sequential image frames are achievable from the monocular camera, existing studies~\cite{wang2019recurrent,zhang2019exploiting,patil2020don} start paying greater attention to the depth estimation under the multi-frame setting. 
% On the other hand, noting that sequential image frames are achievable from monocular cameras, existing 
% Noting that temporal sequential image frames are achievable from monocular cameras, existing
% researches~\cite{wang2019recurrent,zhang2019exploiting,patil2020don} have devoted more attention to the depth estimation in multi-frame setting. 
Inspired by the stereo matching task, multi-frame monocular depth estimation works typically employed the cost volume or cost map~\cite{watson2021temporal,gu2023dro,bae2022multi} to accomplish geometric reasoning and have gradually achieved state-of-the-art performance.
% succeeded in achieving the state-of-the-art.see regions marked by white arrows.
\begin{figure}[t]      
    \centering
    \includegraphics[width =0.48\textwidth]{Images/F1.pdf}
    \vspace{-2mm}
    \caption{Given input images, our CTA-Depth with CTA-Refiner predicts more accurate depth maps compared to the initial prediction, especially for dynamic objects.
    }
    \vspace{-4mm}
    \label{fig:teaser}
\end{figure}

However, the widely applied static scene assumption \cite{klingner2020self,li2019learning} for the construction of the cost volume does not always hold in real-world scenarios.
Specifically, moving objects such as cars, trains and pedestrians result in feature inconsistency deviation, misaligned cost values and degraded re-projection loss, which would mislead the optimization algorithm. 
To address this issue, recent works~\cite{lee2021learning,feng2022disentangling,wimbauer2021monorec} attempted to solve dynamic problems by introducing an auxiliary object motion prediction module and segmentation masks to predict or disentangle dynamic objects explicitly.
It inevitably increases the complexity and redundancy of the model and ignores the sustained temporal relation modeling of moving objects across long-range multiple frames, which thus limits the potential of sequential images for time-crucial industry implementation. 

%They lack the effective prior for dynamic objects to capture the moving objects of long-range frames.
%it is under-estimated with the expert knowledge for learning temporal geometric constraints at the feature level and potential of the recurrent architecture, which limits the further exploration specifically for the dynamic objects in the depth estimation task.
%learn temporal geometric constraints between moving objects

Thus, to efficiently boost the multi-frame context-temporal feature integration for dynamic targets without explicit auxiliary modules, we propose our \textbf{CTA-Depth}, a \textbf{C}ontext-aware \textbf{T}emporal \textbf{A}ttention network for joint multi-frame monocular \textbf{Depth} and pose estimation.
%which avoids the explicit object motion prediction or disentanglement module.
Specifically, we first utilize the multi-level attention enhancement (MAE) module for reliable initial estimation, which applies cross-scale attention layers to achieve ample interaction of different-scale features to equip the network with both local and global attentions.
%-------------------
Furthermore, we develop the refiner CTA-Refiner to iteratively optimize our predictions with the inputs of context and temporal features. In specific, we develop our depth-pose context-aware temporal attention (CTA) with the cross-attention mechanism that assigns the temporal features as values, and the context features as queries and keys.
As a result, it implicitly interacts with the context and temporal features to maintain the estimation integrity of moving objects across multiple sample frames.
Additionally, to expand the temporal field of interest and aggregate useful clues for geometry reasoning, especially for dynamic targets within distant frames, we present our long-range geometry embedding (LGE) and provide it to the CTA process for seizing the long-range temporal geometry prior.

Qualitatively, as shown in Fig.~\ref{fig:teaser}(b), it is difficult for the single-frame method to recover the complete geometry of moving objects, while the predictions from our implicit CTA-Depth in Fig.~\ref{fig:teaser}(c) demonstrate its robustness at high-level feature recognition. Quantitatively, we conduct extensive experiments on three challenging benchmarks to validate the effectiveness of our pipeline against state-of-the-art models. 
% Please see the experiments section for more detailed comparisons.
We summarize our contributions as follows:
\begin{itemize}
    \item  We propose our CTA-Depth, an implicit, long-range Context-aware Temporal Attention guided network for supervised multi-frame monocular depth estimation, focusing on the dynamic object areas. It achieves state-of-the-art performance on challenging KITTI, VKITTI2, and nuScenes datasets.
    % which strengthens the long-range temporal and context interaction with the context-aware temporal attention and long-range geometry embedding module.

    \item  We design a novel depth-pose context-aware temporal attention (CTA), which implicitly learns the temporal geometric constraints for moving objects via attention-based integration. 
    % It achieves the feature consistency and estimation integrity for moving objects, without additional explicit motion prediction or disentanglement module.

    \item We introduce a novel long-range geometry embedding (LGE) module to promote geometry reasoning among the long-range temporal frames.

    \item We develop an effective multi-level attention enhancement (MAE) module to make global-aware initial depth and estimations. It promotes the distinction of far-away small objects from the static background.
    % which injects cross-scale attention layers to enhance the interaction of multi-scale features, thus 
    
    % \item Our CTA-Depth pipeline achieves the state-of-the-art performance on challenging KITTI, VKITTI2, and nuScenes datasets.

\end{itemize}





\if 0
\new{Monocular depth estimation is the task of predicting an accurate depth value (distance relative to the camera) of each pixel from RGB images captured by a monocular camera.
Due to its relatively low cost, small sensor size, and rich content of acquired information, monocular depth estimation has promising prospects for practical applications~\cite{li2022densely,9922174,mumuni2022bayesian}. Given the fact that temporal and spatially continuous images are available in most real-world scenarios, multi-frame monocular depth estimation methods~\cite{wang2019recurrent,zhang2019exploiting,patil2020don} are proposed to utilize the temporally neighboring frames and explore recurrent networks to improve the depth prediction accuracy. Inspired by stereo match tasks, multi-frame works adopted the cost volume~\cite{watson2021temporal,gu2023dro} or cost map  to enable the geometric reasoning through temporally neighboring images and achieved state-of-the-art depth prediction performance.}


 \new{However, the construction of the cost volume and cost map heavily relies on the static scene assumption~\cite{klingner2020self,li2019learning}, which does not always hold for most real-world scenarios. Taking multi-frame image sequences as input, moving objects like cars, trains and pedestrians will violate this assumption and even cause the occlusion problems. 
 The cost volume and loss values in the dynamic object areas are incapable of reflecting the quality of depth hypothesis and prediction, thus misleading the model training. While cost volume based methods perform inaccurate depth prediction on the dynamic object regions, existing works~\cite{lee2021learning,feng2022disentangling,wimbauer2021monorec} have limited success in solving this problem. We argue two reasons accounting for the unsatisfactory performance: \romannumeral1, They attempted to solve the mismatch problem by introducing an auxiliary object motion prediction module to explicitly predict or disentangle dynamic objects, which increased the model complexity and redundancy. \romannumeral2, Expert knowledge for learning temporal geometric constraints at the feature level and exploiting the potential of recurrent network is under-estimated, which limits the performance of the depth estimation model for dynamic objects.}

% Recently, cost-volume-based works \cite{teed2019deepv2d,gu2023dro} adopted the cost volume from stereo match tasks to enable the geometric reasoning through temporal image sequences, and achieved state-of-the-art depth prediction performance while not requiring time-consuming recurrent networks.
% However, the construction of the cost volume heavily relies on the static environment assumption, which does not always hold for most real-world scenarios.
% Taking multi-frame image sequences as input, moving objects like cars, trains and pedestrians will violate this assumption and even cause occlusion problems.
% The cost volume and loss values in the dynamic object areas are incapable of reflecting the quality of depth hypothesis and prediction, thus misleading the model training.}

% \lzz{While cost volume based methods perform inaccurate depth prediction on the dynamic object regions, existing works~\cite{klingner2020self,li2019learning,lee2021learning,feng2022disentangling,wimbauer2021monorec} have limited success in solving moving object problems. We argue two reasons accounting for the unsatisfactory performance: \romannumeral1, Most of them attempted to solve the mismatch problem only at the loss function level and introduced an auxiliary object motion prediction module to explicitly predict or disentangle dynamic objects, which increased the model complexity and redundancy. \romannumeral2, Expert knowledge for capturing temporal geometric constraints at the feature level and further exploiting the potential of recurrent network is under-estimated.}

% \new{To optimize depth prediction of dynamic object areas, recent works attempted to ......} \xz{Please write some recent methods that focus on addressing depth prediction on dynamic object areas and discuss the limitations and drawbacks of these works.}

\if 0
Depth estimation is a crucial step towards inferring scene geometry from 2D images. The goal of monocular depth estimation is to predict an accurate depth value (distance relative to the camera) of each pixel from RGB images captured by a monocular camera. Due to its relatively low cost, small sensor size, and rich content of acquired information, the task of monocular depth estimation has promising prospects for practical applications, 
e.g., autonomous driving, robot navigation, to name a few. Yet, predicting highly precise depth from monocular images (static or sequential) is indeed quite challenging mainly due to the following reasons. First, estimating depth from monocular images is an ill-posed inverse problem \cite{yuan2022newcrfs,gu2023dro,guizilini2022multi}. 
%In other words, many 3D scenes observed in the world may correspond to the same 2D plane due to the occlusion issue.
Meanwhile, dynamic scenes with moving objects further complicate the estimation process, since the moving objects in the scene break the continuity between image frames, thus making it difficult for matching and aligning pixels. 
%Other problematic cases include cluttered background, transparent surface, messy environment, etc.
\fi


\if 0
% Comparison with the baseline and CTA-Depth. Our model with CTA predicts more accurate and smoother depth, especially for moving objects.}
% \caption{Compared to the multi-frame state-of-the-art (DRO) baseline (b), our CTA-Depth (c) with context-aware temporal attention predicts more accurate depth map, especially for moving objects; see regions marked by white arrows.}
% \cite{xu2017multi,hao2018detail,xu2018structured,hu2019revisiting,wang2015towards,huynh2020guiding,ummenhofer2017demon,lee2019big,guizilini20203d} current monocular supervised depth estimation methods can be divided into two types.
To handle this challenging yet important task, there are two main types of monocular depth estimation methods. On the one hand, most depth estimation efforts have been devoted to directly regress the depth maps by designing complex and powerful deep neural networks \cite{eigen2014depth,bhat2021adabins,aich2021bidirectional,lee2019big,fu2018deep,lee2021patch}. On the other hand, many self-supervised learning based works leveraged geometric relationships between multi-frame images via feature matching and predicted the relative camera poses to facilitate the %depth estimation
model training \cite{zhou2017sfm,guizilini20203d, guizilini2022multi}. 
%We follow this idea and take the path of the refinement and optimization of both depth maps and poses, since solving pose and depth is a chicken-and-egg problem. The work of \cite{zhou2017sfm} learned to regress the depth of reference image, whilst predicting the relative camera poses of multiple frames relative to the reference image to improve depth estimation. 
Further, two recent supervised works \cite{teed2019deepv2d,gu2023dro} adopted the cost volume (or cost map) from stereo match tasks to enable the geometric reasoning through temporal image sequences and optimized depth and pose alternately through iterations.
%and  in the network prediction level. 
% introduced an iterative optimization strategy to optimize depth and pose alternately through iterations.
%To solve the optimization problem of depth and pose, \cite{gu2023dro} proposed a deep recurrent optimizer (DRO) with the key idea of updating depth and pose alternately through iterations. %
However, this group of methods often rely on static scene assumption, where local evidences based cost map or cost volume is used for depth and pose refinements, thus being prone to failure for some moving object regions in video frames.
\fi
%suffer from the limitation of inaccurate depth estimation at moving objects due to XX.
%need to predict the relationship between multiple frames, and moving objects will interfere with the relationship prediction, so  cannot handle moving objects well.
%since the focus of DRO is on the network optimization and the usage of the cost map, it has a major limitation of inaccurate depth estimation at moving objects.

% To address this challenging yet extremely important task, monocular depth estimation methods recently started to gain popularity by using deep neural networks. 
%Existing works can be divided into three categories, supervised \cite{fu2018deep,tang2018ba,teed2019deepv2d,lee2020multi,guizilini20203d,guizilini2021sparse,bhat2021adabins,gu2023dro,ranftl2021vision,lee2021patch,patil2022p3depth,yuan2022newcrfs}, unsupervised \cite{zhou2017sfm,chen2019glnet,Godard2019monodepth,ranjan2019competitive,guizilini20203d,gu2023dro} and semi-supervised monocular depth estimation \cite{Kuznietsov2017semi, amiri2019semi} depending on whether the ground-truth depth maps are provided for learning during training.
% \TODO{Brihttps://www.overleaf.com/project/62e3925056ddcb67a282da12efly summarize existing monocular depth estimation works. It is better to organize existing works into several categories. For example, one category of supervised methods, one category of self-supervised method, etc. No need to introduce each work one by one, just group them into categories and then describe each category's key idea. Note: do not repeat the texts in RW section. For this paragraph, it should be a summary of RW section.}


%With the rise of deep learning, CNN and transformer based approaches \cite{Kuznietsov2017semi}\cite{fu2018deep}\cite{Godard2019monodepth}\cite{ranjan2019cc}\cite{lee2019big}\cite{bhat2021adabins}\cite{ranftl2021vision}\cite{yang2021transformers} have shown promising results in monocular depth estimation work. Considering RGB image data from a single view-point as input, these methods typically treated monocular depth estimation as a regression task for a pixel-level depth map. For example, methods like SFMLearner \cite{zhou2017sfm} learn to regress the depth whilst predicting the relative pose since solving pose and depth is a chicken-and-egg problem. However, without an optimization process, those methods are limited by the inability of refining depth estimation.

%More recently, the optimizer-based method (DRO) \cite{gu2023dro} has dominated the task of depth estimation. Unlike the regression-based method, the optimizer iteratively updates the depth map concerning the feature-metric loss defined with multi-view constraints. Specifically, the optimizer takes an expressive feature as inputs and predicts the relative depth variation whereby the feature-metric loss is minimized. Thus, the key for optimizer to learn the accurate depth is the expressive input feature. Motivated by this, DRO utilized convolution layers to enhance expressiveness.
% to enable an accurate monocular depth estimation and 

%In this work, to resolve the ambiguity of dynamic scenes with moving objects and enable an accurate monocular depth estimation, In this way, the extracted features can encode non-local spatial-aware information.

\new{Pursuing accurate depth prediction on dynamic object areas from a more essential feature level and without additional explicit object motion prediction or disentanglement module, we propose CTA-Depth, a supervised spatial-temporal depth estimation framework. Specifically, we first design a multi-level spatial-attention predictor for reliable initial depth prediction, where we employ spatial-attention layers to fuse multi-scale features based on feature encoder. Importantly, to learn the temporal geometric constraints of dynamic objects in multi-frame images, we design a context-aware temporal attention (CTA) mechanism, which learns the value from the temporal features of the sequential temporal frames whilst calculating the key and query from the context features of the current frame. Further, we introduce our CTA into the refinement network to build the CTA-Refiner module to guide the optimization towards the accurate prediction. 
Surprisingly, this CTA-Refiner achieves a significant performance improvement by leveraging the potential of temporal information; see Table~\ref{tableAblationStudy} for the ablation results. }
%Specifically, we present CTA-Depth, a novel multi-frame monocular network for depth estimation.Further, we introduce our CTA into the refinement network to build the CTA-Refiner module, which consists of two sub-modules for depth and pose refinement, respectively. These two sub-modules have similar architecture, with the key insight of taking advantage of CTA to provide more temporal information of the multi-frame inputs to guide the optimization towards the accurate prediction. 
% \new{Pursuing accurate depth prediction on dynamic object areas by recurrent networks and without redundant object motion prediction module,} we propose \new{CTA-Depth, a supervised temporal depth estimation framework that fully explores} the information in temporal domain by using attention to make up the lack of neighborhood information in spatial domain.
% \lzz{Our key insight is to first predict an sub-optimal initial depth and camera poses, and then alternately refine them by effectively injecting our designed context-aware temporal attention (CTA) into the depth-pose recurrent network to provide more temporal information of the multi-frame inputs to guide the optimization.}
% %Specifically, we present CTA-Depth, a novel multi-frame monocular network for depth estimation.


%

%for moving objects and compensate for the lack of spatial neighborhood information in monocular images, we first exploit a context-aware temporal attention (CTA) mechanism. In order to incorporate the temporal context from the sequential frames into the current input feature, our temporal attention layer learns 


%Then we design a multi-level attention enhanced predictor (MAEP) for reliable initial depth prediction, where we employ spatial-attention layers to fuse multi-level features based on feature encoder. In this way, the extracted features can encode non-local context information.
%features and efficient multi-level feature fusion is realized based on the multi-level feature outputs of the transformer encoder.
%%Note that, given a reference image and its neighboring sequential frames, designing an effective transformer based network is non-trivial, since how to properly utilize and incorporate these multiple input frames is still an open problem. 

% \begin{figure*}[t] 
% 	\centering
% 	%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% 	\includegraphics[width =0.9\textwidth]{Images/teaser03.pdf}
% % 	\vspace*{-2mm}
% 	\caption{An illustration of our proposed TA-Opt and the visual comparison between DRO~\cite{gu2023dro} and our method. Obviously, the depth map produced by our network is more accurate, especially on some difficult regions like the transparent windows as pointed by the white arrows and moving objects.}
% \label{fig:teaser}
% \end{figure*}

% 	\vspace*{-2mm}	
% 	\caption{An illustration of the key ideas of our proposed TA-Opt and the visual comparison between DRO~\cite{gu2023dro} and our method. Obviously, the depth map produced by our network is more accurate, especially on some difficult regions like the transparent windows as pointed by the white arrows.}
%  Compared with the DRO baseline (b) without temporal attention,
Extensive experiments on public benchmark datasets validate the effectiveness and superiority of our CTA-Depth compared to existing works. Fig.~\ref{fig:teaser} shows two example results, where the baseline (b) is the recent multi-frame state-of-the-art method \cite{gu2023dro}. Clearly, our method (c) yields more accurate and smoother depth maps, especially on the dynamic regions with moving objects 
%and cluttered background
as pointed by the white arrows. Overall, we summarize the main contributions as follows: 
% More quantitative and qualitative results are illustrated in Section~\nameref{sec:experiments}
%[leftmargin=*]
% long-range dependencies in sequential inputs

% \begin{itemize}
% \item We propose a novel CTA-Depth, where we first design a multi-level attention enhanced predictor to obtain more accurate initial predictions of depth and pose. The enhanced predictor integrates non-local context information from raw inputs via the multi-level feature encoder and spatial-attention layers.
% 	\item  We design 
% 	%CTA-Depth
% 	CTA-Refiner, in which a novel context-aware temporal attention fully explores temporal information and captures long-range feature dependencies of sequential images for reliable depth and pose refinements. %The performance gain proves that our method predicts more accurate and smoother depth for moving objects.
% % 	proves that employing information in temporal domain can make up the lack of neighborhood information in spatial domain.
% 	\item We conduct extensive experiments to demonstrate that our CTA-Depth leads to state-of-the-art performance on KITTI, VKITTI2, and nuScenes datasets.

% \end{itemize}

\begin{itemize}
	\item  \new{We propose a  supervised multi-frame depth estimation model that leverage the information in temporal domain to make up the lack of neighborhood information in spatial domain in monocular images. }
% 	proves that employing information in temporal domain can make up the lack of neighborhood information in spatial domain.
	\item \new{We design a novel depth-pose context-aware temporal attention (CTA) to implicitly learn temporal geometric constraints between moving objects and static scenes in multi-frame images, and we effectively inject the CTA into the recurrent network to achieve accurate prediction on dynamic regions without additional explicit object motion prediction or disentanglement module.}
        \item \new{We propose the spatial-aware multi-level attention enhanced predictor (MSAP) to obtain more accurate initial estimation, which injects spatial attention layers to enhance the interaction of multi-scale features, thus promotes better distinguishment from from far-away small objects to the static background.}
	\item \new{We build a novel supervised spatial-temporal network for multi-frame  monocular depth estimation network and conduct extensive experiments to demonstrate that our CTA-Depth leads to state-of-the-art performance on KITTI, VKITTI2, and nuScenes datasets.}

 % at the feature level obtain more reliable initial predictions of depth and pose. Unlike traditional CNN-based initial predictors, our enhanced predictor integrates non-local context information from raw inputs via the multi-level feature encoder and spatial-attention layers.}
	% \item \lzz{We build a novel supervised multi-frame monocular depth estimation network and conduct extensive experiments to demonstrate that our CTA-Depth leads to state-of-the-art performance on KITTI, VKITTI2, and nuScenes datasets.}

\end{itemize}

% 	\item We propose a novel \textbf{TA-Opt} module that captures long-range feature dependencies of sequential input images for depth and pose refinements. Compared with standard gated recurrent unit (GRU) optimizer, our TA-Opt yields more robust optimization results in problematic cases, such as occlusions, moving objects, reflective surfaces, etc.
% 	\item We design a novel \textbf{TransIDP} block to obtain more robust initial depth prediction. Unlike traditional CNN-based initial depth predictors, our TransIDP integrates non-local context information from raw inputs via the swin-transformer encoder and spatial-attention layers.
% 	\item  We formulate a new method named \textbf{TA-Opt} for monocular depth estimation, which consists of a lightweight scheme \textbf{TA-Opt-A} and a performance-optimal scheme \textbf{TA-Opt-B}.  Extensive experiments on various benchmark datasets demonstrate that both of our proposed solutions outperform others in monocular depth estimation with a significant margin.
	
% 	\item We formulate a novel network named \textbf{TA-Opt} for robust monocular depth estimation, in which we first design a novel \textbf{TransIDP} module for robust initial depth prediction via transformer encoder and spatial-attention layers.
% 	\item We also design a novel \textbf{TA-Opt} module for depth and pose refinements. Compared with standard gated recurrent unit (GRU) optimizer, our \textbf{TA-Opt} considers global context information from raw inputs, thus resulting in more robust optimization results.
% 	\item We conduct extensive experiments on various benchmark datasets and demonstrate that our \textbf{TA-Opt} outperforms others in terms of depth estimation with a significant margin.


%Nevertheless, we argue that the input feature of the optimizer in DRO still has limited context. 
%The main reason is that convolution layers have a limited receptive field size, while global context is critical for depth estimation. In this works, as shown in Figure \ref{fig_first01}, we propose to address this limitation with our multi-frame feature aggregation (MFA) module, where we develop an attention mechanism to enhance the global context of input features. 
%As shown in our experiments, we achieve state-of-the-art performance with the resultant MFA-Depth network.
%The natural solution to the attention is utilizing the recent popular self-attention to incorporate global context. 
%However, we discover that self-attention harms the optimization process in this work. The reason is that the input feature of the optimizer consists of feature-metric cost map and depth map which are dynamic in iterative process, causing the challenges in defining the attention between pixels.

%Instead, our attention defines the attention matrix and value matrix in heterogeneous feature spaces. Specifically, unlike the vanilla self-attention that calculates the key, query, and value matrix from the same input feature, we learn value matrix from the input feature but estimate the key and query matrix from a new context feature. Note that the context feature excludes the dynamic depth and feature-metric cost maps. In this case, we define the attention matrix in new static feature space to achieve meaningful visual similarity. 
%Experimentally, we observe that, different from the vanilla self-attention that fails to work in the optimizer process, our attention mechanism significantly improves the performance.

\fi

\begin{figure*}[!t]  
        \centering
	\includegraphics[width =0.98 \textwidth]{Images/F2.pdf}
	\caption{
		Overview of our CTA-Depth. Given a reference image $I_r$ and its $N$ monocular sequential images $\{I_i\}_{i=1}^N$, we first group $N$ pairs of network inputs, where each pair is composed of $I_r$ and a sequential image $I_i$. We then feed the two images into the MAE module and go through two heads to obtain the initial depth $D_r^0$ ,and pose $P_i^0$. Hence, the CTA-Refiner is proposed to alternately update the depth map and pose through iterations until the optimum solution, $D_r^*$ and $P_i^*$. In particular, with multiple temporal-neighboring frames $I_j$, we also design a long-range geometry embedding module to provide long-range temporal geometric priors for the depth refiner efficiently.
	}
	\vspace{-2mm}
    \label{fig:overview}
\end{figure*}

==> method.tex <==
\section{Method}
\label{sec:method}



\subsection{Overview}

We demonstrate the framework of our approach in Fig.~\ref{fig:overview}, which mainly consists of five components: the network inputs, the multi-level attention enhancement (MAE) module, the depth \& pose context net, and the context-aware temporal attention refiner (CTA-Refiner) which includes the depth-pose context-aware temporal attention (CTA) module and the last long-range geometry embedding (LGE) module.

Given a reference image $I_r$ within one video captured via a monocular camera, and its $N$ video frames $\{I_i\}_{i=1}^N$, our goal is to predict the $I_r$'s accurate depth $D_r^*$ and the relative camera poses $\{P_i^*\}_{i=1}^N$ for sequence image $I_i$ with respect to $I_r$.
Specifically, we first regard the monocular video frames as network inputs. 
Then, we adopt the multi-level attention enhancement (MAE) module to extract representative visual features for the following depth head and (shared) pose head, which produces the initial depth $D_r^0$ and initial pose $P^0$.
Meanwhile, we employ the depth \& pose context net to extract context features $F_r^c$ for depth and $F_i^c$ for pose.
In addition, the long-range geometry embedding module seizes the multi-frame temporal geometry knowledge to create the long-range geometry embedding (LGE) $\varphi(F_j)$, which is further provided to the CTA to assist the refinement.
Afterwards, we adopt the context-aware temporal attention refiner (CTA-Refiner) to alternately update the predicted depth map and camera pose, which gradually converges to the optimal depth $D_r^*$ and pose $P_i^*$.
% where we manage to design the depth-pose context-aware temporal attention (CTA) to strengthen the long-range temporal-context interaction and the feature consistency with the LGE.

%------------old--------------------------------

% We first feed a pair of images (i.e., $I_r$ and $I_i$) into initial predictors to obtain \lzz{reliable} initial depth $D_r^0$ and pose $P_i^0$.
% We then design the \emph{CTA-Refine} to alternately update $D_r^0$ and $P_i^0$ to obtain the final depth $D_r^*$ and pose $P_i^*$.

%
%A recent work named deep recurrent optimizer (DRO)~\cite{gu2023dro} has achieved promising performance with the key idea of alternately updating the depth and camera poses through iterations.
%It is, however, suffers from the limited representative capability of extracted local features.
%To address this issue, we propose to further enhance the network performance by introducing the transformer mechanism~\cite{Vaswani2017attention}.

%

%
% Fig.~\ref{fig:overview} shows the detailed architecture. 
%

%transformer-enhanced features $F_r^A$ and $F_i^A$

% 
 
%
%
%At last, we design the \emph{CTA-Refine} to alternately update the predicted depth map and camera pose to obtain the final depth $D_r^*$ and pose $P_i^*$.



%The architecture overview is shown in Figure\ref{fig002}. And a more detailed diagram of our MFA-Depth abstraction about a single GRU module is shown in Figure \ref{fig003}. In DRO \cite{gu2023dro}, two iterative optimizers alternately update the depth and camera poses through iterations to minimize a feature-metric cost based on multiple video frames. However, DRO used local CNN features that suffer from the problem of the limited receptive field. To address this issue, we apply the transformer \cite{Vaswani2017attention} to solve this problem.

%In the self-attention mechanism of transformers, there are query, key, and value mappings from the same input feature vector. Unlike the general self-attention, based on the context network, we use query and key mappings on a context feature map to model the appearance of self-similarities in the reference image. Based on the feature network, we use value mappings on input features of depth or pose. The attention matrix computed from the query and key features can aggregate the value features. We name it a Multi-Frame Feature Aggregation (MFA) module. As shown in Figure \ref{fig004}, the MFA module can aggregate the input features with the context features and generate feature vectors to be fed into the GRU module.

%\begin{figure}[htp]      
%	\centering
%	\center{\includegraphics[width =0.48 \textwidth]{Images/MFA_FIGURE_002.jpg}}
%	\caption{The detailed diagram of our MFA module. "$\bigotimes$" denotes matrix multiplication, and "$\bigoplus$" denotes element-wise sum. Query mapping and key mapping are performed on context features and value mapping is performed on input features. }
%	\label{fig004}
%\end{figure}

%As shown in Figure \ref{fig002}, our method outputs the depth of the reference image and the relative camera poses based on a reference image and $N$ sequential images from multiple video frames. The input images are passed through a shared feature network to yield a feature map. Then the depth and pose context networks are used. A depth head and a pose head output an initial depth map and initial relative poses with these features. These initial results are iteratively refined by the depth GRU module and the pose GRU module alternately based on our MFA modules. Subsequently, the depth GRU and pose GRU networks output the final results.

\begin{figure}[t]        
	\center{\includegraphics[width =0.48\textwidth]{Images/F3_2.pdf}}
	\vspace{-2mm}
	\caption{The architecture of our multi-level attention enhancement (MAE) module, which adequately integrates multi-level image features via feature encoders, cross-scale attention layers, and PPM module. 
    ``$R$" denotes the rearranged up-scaling for feature maps.
    % Between each cross-attention layer, the rearrange upscale "$R$" is performed for feature map up-scaling.
	}
	\vspace{-2mm}
	\label{fig:encoder}
\end{figure}

\subsection{Multi-level Attention Enhancement (MAE)}
\label{subsec:embed}
Affiliated with the optimizer-based pipeline, we deliver our multi-level attention enhancement (MAE) module to achieve the initial prediction of depth and pose.
As shown in Fig.~\ref{fig:encoder}, we propose the multi-level feature setting and pyramid pooling module to reinforce the interest of the far-away small targets. 
In addition, to distinguish distant moving objects from the static background, we adopt cross-scale attention layers to enhance the interaction of different-scale features.
% Our proposed non-local cooperation 

Specifically, as shown in Fig.~\ref{fig:encoder}, we utilize the feature encoder to extract four different-scale features from $I_r$.
The low-level features focus on the local details, while the high-level features seize the global context information, which both contribute to the rising interest of the distant targets~\cite{lin2017feature,liu2018path}.
Afterwards, we employ the pyramid pooling module (PPM)~\cite{zhao2017pyramid} to aggregate these features and deliver four cross-scale attention layers to fuse the multi-level feature maps.
We use the scaled features $F_i$ as the query and key, and adopt the fusion features $F_j$ as the value to stimulate the interaction of multi-scale features. Within each cross-attention layer, we also introduce the rearranged up-scaling operation \cite{yuan2022newcrfs} to reduce the network complexity and boundary contour refinements. As shown in Fig.~\ref{fig005}, our method achieves accurate depth prediction of objects at different scales and long distances.
% Within each cross-attention layer, we also introduce the \gyz{rearrange up-scaling operation for feature up-scaling}, so that we could achieve robust context features for initial depth and pose prediction.  


% As above, but adding the rearrange upscale to reduce the parameters of the network. This module visually sharpens the boundary contours, though it does not achieve a large performance gain. Then the PPM is used to aggregate the non-local information of the whole image and consequently enhances the performance.


\begin{figure}[t]        
	\center{\includegraphics[width =0.48\textwidth]{Images/F4-new.pdf}}
	\caption{
		Illustration of the Depth/Pose CTA. Our CTA-Refiner alternately optimizes the depth and the pose. During the depth refinement, the depth CTA uses the depth context feature $F_r^c$, the temporal feature $F_r^t$, and the Long-Range GE as inputs and feeds the outputs into the depth GRU. For the pose refinement, the pose CTA employs the pose context-aware feature $F_i^c$, the temporal feature $F_i^t$ and the Long-Range GE as inputs, then its outputs are fed into pose GRU.}
		\vspace{-2mm}
	\label{fig:optimizer}
\end{figure}

% \begin{figure}[t]        
% 	\center{\includegraphics[width =0.48\textwidth]{Images/F4.pdf}}
% 	\caption{
% 		Illustration of the Depth/Pose CTA. Given the initial depth $D_r^0$ and relative camera pose $P_i^0$, CTA-Refiner alternately optimizes the depth or the pose. During the depth refinement (solid line), we first compute a cost map from the current solution $D_r^t$ and $P_i^t$, and extract depth temporal features $F_r^t$. Note that this $F_r^t$ contains the multi-frame temporal information from reference image $I_r$ and temporal sequential images $I_i$, since its inputs $D_r^t$ and $P_i^t$ are derived from $I_r$ and $I_i$. Then $F_r^t$ and the depth context features $F_r^c$ are fed into our depth context-aware temporal attention together. For the pose refinement (dashed line), we extract the pose temporal features $F_i^t$ and feed $F_i^t$ into the pose context-aware temporal attention along with the pose context features $F_i^c$.}
% 		\vspace{-2mm}
% 	\label{fig:optimizer}
% \end{figure}

\subsection{Context-aware Temporal Attention (CTA)}
\paragraph{CTA-Refiner}
We adopt the CTA-Refiner to iteratively refine initial estimations to the final converged depth $D_r^*$ and pose $P_i^*$, together with two introduced extra inputs: the context features $F_r^c$ for depth and $F_i^c$ for the pose from the depth \& pose context net, 
The refiner accepts these inputs to produce the prediction offset $\Delta D_r^t$ and $\Delta P_i^t$ and then updates the depth and pose as follows: 
\begin{align}
    D_r^{t+1} \leftarrow D_r^t + \Delta D_r^t, \\
    P_i^{t+1} \leftarrow P_i^t + \Delta P_i^t.
\end{align}
In detail, we first calculate the cost map given $D_r^t$, $P_i^t$, $F_r$ and $F_i$, as shown in Fig.~\ref{fig:overview}, where optimization for pose remains freezing when optimizing depth, and vice versa.
Notably, the cost map measures the distance in feature space between $I_r$ and the sequence image $I_i$.
Next, we adopt a simple feature extractor (two convolutions) to obtain the temporal features $F_r^t$ from the cost map, preparing for the following depth-pose CTA. 
Thus it implicitly rectifies the implied content-temporal inconsistency for moving objects and effectively promotes information integration between temporal features and depth-pose context features.

We formulate the cost map as the $L2$ distance between aligned feature maps $\mathcal{F}$. Given the depth map $D$ of the reference image
$I_r$ and the relative camera pose $T_i$ of another image $I_i$ with respect to $I_r$, the cost is constructed at each pixel $x$ in the reference image $I_r$:
\begin{equation}
	\mathbf{C}_{i}(x)=\left\|\mathcal{F}_{i}\left(\pi\left(\mathbf{T}_{i} \circ \pi^{-1}(x, \mathbf{D}(x))\right)\right)-\mathcal{F}_{r}(x)\right\|_{2},
\end{equation} 
where ${\pi()}$ is the projection of 3D points in 3D space onto the image plane and ${\pi^{-1}(x,{D}(x))}$ is the inverse projection. The transformation converts 3D points from the camera space of $I_r$ to that of $I_i$. The multiple cost values are averaged at each pixel ${x}$ for multiple neighboring images.

\paragraph{Depth-pose Context-aware Temporal Attention (CTA)} 
The construction of the cost volume heavily relies on the static scene assumption, where it supposes that the object points remain static at time $t$ and $t^*$.
Thus, we re-project the features at time $t$ to another plane with pose $t^*$ at time $t^*$, to achieve the matching cost values.
However, moving objects break this assumption since targets such as cars, trains, or pedestrians with a certain speed could move within the time gap.
This gives rise to the feature inconsistency deviation, degraded (mismatching) cost values and re-projection loss, and finally drawbacks our optimization for depth and pose. 
We discard explicit settings such as the object motion prediction module or disentangle module~\cite{lee2021learning,feng2022disentangling,wimbauer2021monorec}, which brings additional complexity and ignores the potential of complementary context-temporal information.
Instead, we deliver our context-aware temporal attention (CTA) to implicitly rectify the mismatching problem, which efficiently cooperates the temporal features with context features via attention-based communication to achieve the feature consistency and estimation integrity.

%-----------------------------
Specifically, as shown in Fig.~\ref{fig:optimizer}, taking depth optimization as 
an example, we first lift the temporal feature $F_r^t$ to value ($V$) vectors via the mapping function $\sigma(\cdot)$.
Meanwhile, we create query ($Q$) and key ($K$) vectors by adding the mapping functions $\theta(\cdot)$ and $\phi(\cdot)$ from the context feature $F_r^c$, and prepare long-range geometry embedding (LGE). 
We first allocate the query, key and value as  $Q = \theta(F_r^c)\oplus LGE, \  K = \phi(F_r^c)\oplus LGE$, and $V= \sigma(F_r^t)$, respectively.
Subsequently, the depth context-aware temporal attention is denoted as follows:
\begin{align}
F_r^d  = f_{\text{s}}(Q\otimes K)\otimes V \oplus F_r^t,
\end{align}

% \begin{equation}
% \label{equ:attention1}
% F_r^d = f_{\text{s}}((\theta(F_r^c)\oplus LGE)\otimes(\phi(F_r^c) \oplus LGE))\otimes\sigma(F_r^t) \oplus F_r^t,
% \end{equation}
where $f_s$ denotes the softmax operation, $\oplus$ denotes the point-wise addition and $\otimes$ denotes matrix multiplication. 

Intuitively, compared with directly feeding $F_r^t$ and $F_r^c$ for refinement, our CTA explicitly aligns the features for moving objects through the cross-attention mechanism, to compensate for the mismatching discrepancy, which guarantees temporal-context feature fusion and seamless depth refinement.
The temporal feature also helps the context feature to fulfill the moving target’s integrity, such as the second row of Fig.~\ref{fig:teaser}, where we rectify the wrong estimation in the ‘hole’ of the car head with temporal-content interaction.
Similarly, for the pose optimization with fixed depth optimization, we employ context features $F_i^c$ to extract query ($Q$) and key ($K$) vectors with added LGE.
Hence, we allocate the query, key and value as $Q = \theta(F_i^c)\oplus LGE, \   K = \phi(F_i^c)\oplus LGE$, and $ V= \sigma(F_i^t)$, respectively.
Particularly, we lift the temporal feature $F_i^t$ for value ($V$) vectors and finally adopt similar attention for pose context-aware temporal attention:
\begin{align}
F_i^p  = f_{\text{s}}(Q\otimes K)\otimes V \oplus F_i^t.
\end{align}
% \textcolor{red}{TOO LONG, SEPARATE THE FUNCTION INTO TWO}
% \begin{equation}
% \label{equ:attention2}
% F_i^d = f_{\text{s}}((\theta(F_i^c) \oplus LGE )\otimes (\phi(F_i^c) \oplus LGE ))\otimes\sigma(F_i^t) \oplus F_i^t.
% \end{equation}
%-------------------------
\subsection{Long-range Geometry Embedding (LGE)}
Existing works~\cite{gu2023dro,feng2022disentangling} usually adopt the two-frame correlation, such as the cost volume constructed from two frames, which limits the temporal interest field and wastes temporal helpful clues for geometry reasoning within the originally long-range multiple frames.
Therefore, to expand the temporal geometry relation range, especially for moving targets within long-range frames, we present our long-range geometry embedding module to create long-range geometry embedding (LGE), which seizes the beneficial long-range temporal hints for geometry and is inserted into the depth-pose CTA to promote the present depth and pose refinement.

Specifically, we demonstrate the detailed structure in Fig.~\ref{fig:overview}, where we build the long-range cost map with the reference frame $I_r$ and another arbitrary frame $I_j (j\neq{i})$.
Hence, we can achieve N-1 cost maps with N-1 different-range frames.
Notably, we achieve the temporal feature with long-range cost maps and convolution, which reveals the same as the procedure in CTA-Refiner. 
Afterwards, we propose the $1\times1$ Conv, ReLU and Conv to deliver the geometry embedding $\varphi (F_j)$.
Specifically, the number of $\varphi (F_j), j\neq{i}$ is N-1.
Then, we aggregate this long-range temporal knowledge to create our embedding $F_{ge}$ via the addition operation:
\begin{equation}
    F_{ge}=\sum_{j, j\neq i}^{N} \varphi (F_j),
\end{equation}
which will be added to the query and key vectors within the depth-pose CTA.
Our approach efficiently reveals most of the geometry clues within the long-range temporal frames.
It is also regarded as a temporal geometry prior to enhance the temporal-context association process. 


\subsection{Supervised Training Loss}
We train our network by optimizing both depth and pose errors.
Then, we formulate the depth loss as the $L1$ distance between the predicted depth map $D$ and the associated ground truth $\hat{D}$:
\begin{equation}
	\mathcal{L}_{\rm depth} = \sum_{s=1}^m \gamma^{m-s} \Arrowvert { {D}}^s - \hat{ {D}} \Arrowvert_1,
\end{equation}
where the discounting factor $\gamma$ is 0.85 and $s$ denotes the stage number. 
There are $m$ alternating update stages of depth and pose refinements. At each stage, we repeatedly refine the depth and pose $n$ times.
%during recurrent optimization.
Next, our pose loss is defined based on the ground truth depth $\hat{D}$ and pose ${\rm {\hat T}_i}$ with $I_i$ relative to the reference image $I_r$: 
\begin{equation}
\begin{aligned}
	\mathcal{L}_{\rm pose} = &\sum_{s=1}^m\sum_{x} \gamma^{m-s} \Arrowvert \pi({\rm {T}}_i^s \circ \pi^{-1}(x, \hat{D}(x)))\\
	&- \pi({\hat{\rm {T}}}_i \circ \pi^{-1}(x,\hat{D}(x)))  \Arrowvert_1 ,\\
	\end{aligned}
\end{equation}
where $\circ$ means the Hadamard product. 
The pose loss summarizes the re-projection deviation of the pixel $x$ according to the estimated camera pose ${\rm {T}}_i^s$ and the true pose ${\hat{\rm {T}}}_i$ in each stage. 
${\pi()}$ is the projection of 3D points in 3D space onto the image plane. Its inverse projection ${\pi^{-1}(x,\hat{D}(x))}$ maps the pixel ${x}$ and its ground truth depth $\hat{D}(x)$ back points in the 3D space. 
Finally, the total supervised loss is calculated by:
\begin{equation}
	\mathcal{L}_{\rm supervised} = \mathcal{L}_{\rm depth} + \mathcal{L}_{\rm pose} . 
\end{equation}



\if 0
\subsection{CTA-Refiner for Depth and Pose}
\label{subsec:optimizer}
 In this work, we input the pairs of image frames that are time series data. 
 In our CTR-Refiner, this time series data is fully exploited as context-aware temporal information.
 As shown in Fig.~\ref{fig:overview}, after obtaining the predicted depth $D_r^0$ and the predicted pose $P_i^0$, the final step is an iterative refinement of these initial results using our designed CTA-Refiner, and converge to the final depth $D_r^*$ and pose $P_i^*$. 
 The architecture is illustrated in Fig.~\ref{fig:optimizer}. 
 Our CTA-Refiner effectively injects the proposed context-aware temporal attention into the standard gated recurrent unit (GRU) optimizer~\cite{chung2014empirical}. 
In detail, the CTA-Refiner consists of a CTA-Refiner-Depth sub-module 
%(see top blue lines)To be more specific, denote 
and a CTA-Refiner-Pose sub-module, which refines the predicted depth and pose, respectively. 
Note that, during network training, the CTA-Refiner-Depth and CTA-Refiner-Pose work alternately through iterations. 
The updates produced by the GRU optimizer for depth is $\Delta D_r$ and the update for pose is $\Delta P_i$. 
At the $t$-th iteration, we update the depth map and camera pose alternately with $m$ stages. 
At each stage, we first freeze CTA-Refiner-Pose and update the depth using CTA-Refiner-Depth as
\begin{equation}
	D_r^{t+1} \leftarrow D_r^t + \Delta D_r^t,
\end{equation}
which is repeated by $n$ times. 
Then, we freeze CTA-Refiner-Depth and update the relative camera pose using CTA-Refiner-Pose as
\begin{equation}
	P_i^{t+1} \leftarrow P_i^t + \Delta P_i^t,
\end{equation}
which is also repeated by $n$ times.
% In experiments, we follow \cite{gu2023dro} to set $m=3$ and $n=4$.
In experiments, we set $m=3$ and $n=4$ following the baseline method~\cite{gu2023dro}. 
Inside each sub-module, the architecture is similar. 
Here, we only take the CTA-Refiner-Depth (see top of Fig.~\ref{fig:optimizer}) as an example to describe the detailed design. 

We first compute the cost map given $D_r^t$ and $P_i^t$ that are needed to be updated. 
The cost map measures the distance in feature space between $I_r$ and the aligned image $I_i$ using the predicted $D_r^t$ and $P_i^t$. 
Inverse warping is used for computing the cost map. 
Unlike the baseline DRO \cite{gu2023dro} that directly feeds the constructed cost map feature and context feature to the GRU optimizer for minimization, we here propose to extract features $F^t$ from the cost map, which $F_i^t$ for depth and $F_r^t$ for pose.
Then we obtain the adaptive dynamic scene-aware depth features $F_r^d$ or pose features $F_i^p$ via our proposed context-aware temporal attention mechanism. 
Finally, we use GRU to minimize.
Formally, given $F_r^t$ or $F_i^t$, we first employ mapping function $\sigma(\cdot)$ to lift $F_r^t$ or $F_i^t$ to value vectors.
The query and key vectors are obtained from the context features $F_r^c$ or $F_i^c$ via mapping functions $\theta(\cdot)$ and $\phi(\cdot)$, respectively.
% and $[\cdot,\cdot]$ denotes the concatenation operation
Hence, the operation of depth context-aware temporal attention mechanism is
\begin{equation}
	\label{equ:attention1}
	F_r^d = f_{\text{softmax}}(\theta(F_r^c)\otimes\phi(F_r^c))\otimes\sigma(F_r^t)+F_r^t,
\end{equation}
where $\otimes$ denotes matrix multiplication. Similarly, the pose context-aware temporal attention mechanism is
\begin{equation}
	\label{equ:attention2}
	F_i^p = f_{\text{softmax}}(\theta(F_i^c)\otimes\phi(F_i^c))\otimes\sigma(F_i^t)+F_i^t.
\end{equation}

Intuitively, compared with directly feeding $F^t$ and $F^c$ for the refinement, the attention mechanism explicitly injects the original context features $F_r^c$ of $I_r$ and the aggregated features based on attention operation into the optimization process, which provides more information from the reference image and sequential images to guide the depth refinement.
Similarly, for the CTA-Refiner-Pose, besides using $F_i^t$, we further employ context features $F_i^c$ to extract query and key vectors, where $F_i^t$ is extracted from both $I_r$ and $I_i$ as shown in Fig.~\ref{fig:overview}.
In this way, the update of pose not only relies on the features $F^t$ of cost map, but also incorporates the additional information of $F_i$ and the aggregated features based on attention operation.  
Thanks to the attention operation as described in Eq.~\eqref{equ:attention1} and Eq.~\eqref{equ:attention2}, our CTA-Refiner considers more comprehensive information to resolve the ambiguity caused by moving objects when updating, thus making the refined depth (or pose) more accurate.


% \begin{figure*}[t]        
% 	\center{\includegraphics[width =0.98 \textwidth]{Images/optimizer.pdf}}
% 	\caption{
% 		The architecture of our proposed CTA-Refiner to optimize depth (solid line) or pose (dashed line) alternately.
% 		%, consisting of a depth optimization (solid line) and a pose optimization (dashed line) to be updated alternately through iterations. 
% 		Note that, the extracted feature $F^t$ contains the temporal information from both reference image $I_r$ in $t_0$ and sequential image $I_i$ in $t_i$. 
% 		In the right-hand side, $F_r^t$ and $F_r^c$ are for depth attention, while $F_i^t$ and $F_i^c$ are for pose attention.
% 		%In our proposed CTA module, the query and key mapping are performed on context features $F^c$ and value mapping is performed on input feature $F^t$. In detail, we input $F_r^t$ and $F_r^c$ to depth context-aware temporal attention, $F_i^t$ and $F_i^c$ to pose context-aware temporal attention.
% 		}
% % 		In detail, we input $F_r^t$ and $F_r^c$ for depth context-aware temporal attention, $F_i^t$ and $F_i^c$ for pose context-aware temporal attention.
% 	\label{fig:optimizer}
% \end{figure*}

% The architecture of our proposed CTA-Refiner to optimize depth (solid line) or pose (dashed line) alternately. consisting of a depth optimization (solid line) and a pose optimization (dashed line) to be updated alternately through iterations. Note that, the extracted feature $F^t$ contains the temporal information from both reference image $I_r$ in $t_0$ and sequential image $I_i$ in $t_i$. In the right-hand side, $F_r^t$ and $F_r^c$ are for depth attention, while $F_i^t$ and $F_i^c$ are for pose attention.

% \lzz{The architecture design of our CTA-Refine, which consists of a depth optimization process (solid line) and a pose optimization process (dashed line). Note that, these two optimization process work alternately through iterations. The subscript "r" represents the reference image ($t_0$) , and "i" represents the sequential image from a different frame. We input pairs of image frames that are the time series data. In our proposed CTR-Refine module, this time series data is fully exploited as the context-aware temporal information.}

% \caption{
% 		The architecture design of our CTA-Refine, which consists of a CTA-Refine-Depth sub-module and a CTA-Refine-Pose sub-module for depth and pose updating, respectively. %For each sub-module, besides the conventional gated recurrent unit (GRU) optimizer, we further inject the attention mechanism. 
% 		Note that, the CTA-Refine-Depth and the CTA-Refine-Pose work alternately through iterations.
% 	}

% As shown in Fig.~\ref{fig:overview}, \lzz{ the initial predictors (including feature extraction and head) for depth and pose are needed for predicting the initial depth $D_r^0$ and initial pose $P_i^0$. we build a novel multi-level attention enhanced predictor based on feature encoder, pyramid pooling module (PPM) \cite{zhao2017pyramid} and cross-attention layers \cite{Vaswani2017attention}. We have two solutions: CTA-Refine and TA-Opt (L). In TA-Opt, we use the light-weight ResNet18 as feature encoder. In TA-Opt (L), we use the large Swin transformer \cite{liu2021swin} as feature encoder and use cross-attention layers and pyramid pooling module as feature fusion modules for the initial depth predictor. Except the feature encoder, the other modules have the same structures for TA-Opt and TA-Opt (L). Especially, in  TA-Opt (L), the initial depth predictor is independently trained based on supervised learning and it is integrated into the whole framework (also called two-stage cascade) in inference time as shown in Fig.~\ref{fig:teaser}. In  TA-Opt, different from  TA-Opt (L), all modules are trained in a single framework based on supervised learning or self-supervised learning.}

\subsection{Supervised Training Loss}

Our network is trained by evaluating both depth and pose errors.
%Given ground truth, we supervise the training by evaluating the depth and pose errors. 
The depth loss is formulated as the L1 distance between the predicted depth map $D$ and the associated ground truth $\hat{D}$:
% Our method can be applied to both supervised and self-supervised depth estimation. We take the supervised depth estimation as our major task according to our application cases. Given ground truth, we supervise the training by evaluating the depth and pose errors. Depth loss function computes the L1 distance between the predicted depth map D and the ground-truth depth map \^{D} in each stage:
\begin{equation}
	\mathcal{L}_{\rm depth} = \sum_{s=1}^m \gamma^{m-s} \Arrowvert {\rm {D}}^s - \hat{\rm {D}} \Arrowvert_1,
\end{equation}
where the discounting factor $\gamma$ is 0.85 in the experiments and $s$ is the stage number. There are $m$ alternate optimization stages for depth and pose refinements. 
%during recurrent optimization.
The pose loss is defined based on the ground truth depth $\hat{D}$ and pose ${\rm {\hat T}_i}$: 
\begin{equation}
\begin{aligned}
	\mathcal{L}_{\rm pose} = &\sum_{s=1}^m\sum_{x} \gamma^{m-s} \Arrowvert \pi({\rm {T}}_i^s \circ \pi^{-1}(x, \hat{D}(x)))\\
	&- \pi({\hat{\rm {T}}}_i \circ \pi^{-1}(x,\hat{D}(x)))  \Arrowvert_1 .\\
	\end{aligned}
\end{equation}
This pose loss computes the image re-projection of a pixel $x$ according to the estimated camera pose ${\rm {T}}_i^s$ and the true pose ${\hat{\rm {T}}}_i$ in each stage. ${\pi()}$ is the projection of 3D points in 3D space onto the image plane. The final supervised loss is then calculated by:
\begin{equation}
	\mathcal{L}_{\rm supervised} = \mathcal{L}_{\rm depth} + \mathcal{L}_{\rm pose} . 
\end{equation}
\fi


==> rw.tex <==
\section{Related Work}
\label{rel_work}


\paragraph{Monocular Depth Estimation.}
Convolutional neural networks with LiDAR supervision \cite{wang2015towards,fu2018deep,tang2018ba,teed2019deepv2d,lee2020multi,guizilini2021sparse,lee2021patch} have shown promising results in monocular depth estimation. As a pioneer, Eigen et al.~\cite{eigen2014depth} directly regressed depth by employing two stacked deep networks that made a coarse prediction from the whole image and then refined it locally.
On the other hand, \cite{laina2016deeper} adopted an end-to-end single CNN architecture with residual learning. 
To guide the encoded features to the desired depth prediction, \cite{lee2019big} further deployed it with local planar guidance layers. 
Recently, \cite{ranftl2021vision} introduced a dense prediction transformer ~\cite{Vaswani2017attention} for depth prediction. 
Meanwhile, \cite{bhat2021adabins,yang2021transformers} developed global information processing with vision transformer~\cite{dosovitskiy2020image} for performance boost. 
Besides, \cite{yuan2022newcrfs} adopted the swin-transformer \cite{liu2021swin} as the image encoder and the neural window fully-connected conditional random fields (NeWCRFs) module as the feature decoder. 
In particular, inspired by the RAFT \cite{teed2020raft} which employed a GRU-based recurrent operator to update optical flow, \cite{gu2023dro} proposed a multi-frame monocular approach with a deep recurrent optimizer to update the depth and camera poses alternately. However, these cost-map-based multi-frame methods \cite{teed2019deepv2d,gu2023dro} lead to performance degradation within dynamic areas due to the static scene assumption. To solve this problem, we introduce a long-range geometry embedding module and effectively inject the proposed depth-pose context-aware temporal attention into the deep refinement network for the optimization process of depth and pose.

\paragraph{Depth Estimation in Dynamic Environment}  Moving objects significantly hamper the multi-frame matching strategy due to the inevitable object truncation and occlusion.
Specifically, both the re-projection loss calculation and the cost volume construction fall into catastrophic failure cases during the positional change of observed targets. 
Existing works~\cite{li2019learning,lee2021learning,watson2021temporal} thus leveraged the segmentation mask to separate the static-scene depth loss from moving objects.
In particular, they also proposed explicit object motion prediction and a disentanglement module to assist the cost volume construction.
Specifically, SGDepth \cite{klingner2020self} proposed a semantic masking scheme providing guidance to prevent dynamic objects from contaminating the photometric loss. 
DynamicDepth \cite{feng2022disentangling} introduced an object motion disentanglement module that takes dynamic category segmentation masks as input to explicitly disentangle dynamic objects.
Considering time-crucial tasks such as autonomous driving, instead of adopting explicit redundant static-dynamic separation algorithms, we developed an efficient implicit modeling pipeline with our novel context-aware temporal attention module.
Besides, noting that previous works limited their methods to a few frames only due to an increase in computational cost, we developed a novel geometry embedding module to effectively encode semantic guidance from long-range time series. As a result, our pipeline can dynamically interact with the long-range semantic flow with the current-frame spatial geometry in a fully differentiable manner and is thus available for real industry implementation.

% \paragraph{Learning to Optimize.} Most vision based tasks can formulated as the optimization problem. 
% Some efforts such as \cite{amos2017optnet,lv2019taking} have drawn on the power of neural networks to predict the inputs or parameters of the optimizer. 
% In particular, OptNet \cite{amos2017optnet} incorporated the differentiable optimization problem as individual layers in a large trainable network. 
% Then RAFT \cite{teed2020raft} introduced an approach about learning to optimize, which employs a GRU-based update operator to update optical flow recurrently. 
% Building on this development and traditional bundle adjustment algorithm, \cite{gu2023dro} utilized a GRU module as a zeroth-order optimizer embedded in the network that alternately updates the depth and pose. Since this method focuses on the network optimization, it has limited capability of extracting adaptive accurate features and modeling the long-range dependencies and temporal relation. 
% Our method effectively injects the proposed context-aware temporal attention and temporal embedding module into the deep refinement network for the optimization process of depth and pose.


% \vspace{-3mm}
% \paragraph{Transformers for Monocular Depth.} While transformer has emerged as the standard in the NLP community, its application to CV tasks still has unpredictable potential. Wang et al. \cite{wang2018non} introduced non-local operations as a generic family of building blocks for capturing long-range dependencies. This work is beneficial for many CV tasks where the simple addition of non-local blocks can enhance the model's performance. The recent trend in depth estimation has been to combine CNN with vision transformers. 
% \cite{ranftl2021vision} introduced dense prediction transformer (DPT) to effectively leverage vision transformers for depth estimation. Meanwhile, some works \cite{bhat2021adabins,yang2021transformers} proposed transformer-based architectures and used global processing of information on the output of CNN for improving the overall depth estimation based on heavy-weight backbones. Recently, \cite{yuan2022newcrfs} built a bottom-up-top-down structure, where the swin transformer \cite{liu2021swin} serves as the encoder and the neural window fully-connected Conditional Random Fields (NeW CRFs) module serves as the decoder.
% \vspace{-3mm}
% \paragraph{Learning to Optimize.} Various problems in vision can be side-step formulated as an optimization problem. Some efforts such as \cite{amos2017optnet,lv2019taking} have drawn on the power of neural networks to predict the inputs or parameters of the optimizer. In particular, OptNet \cite{amos2017optnet} incorporated the differentiable optimization problem as individual layers in a large trainable network. Then RAFT \cite{teed2020raft} introduced an approach about learning to optimize, which employs a GRU-based update operator to update optical flow recurrently. Building on this development and traditional bundle adjustment algorithm, DRO \cite{gu2023dro} utilized a GRU module as a zeroth-order optimizer embedded in the network that alternately updates the depth and pose. However, since the focus of DRO is on the network optimization, it has limited capability of extracting accurate global features and modeling the long-range dependencies. In our work, \lzz{we effectively inject our proposed context-aware temporal attention into the deep refinement network for optimization process of depth and pose.}


% \lzz{we effectively inject our context-aware temporal attention into the optimization process of depth and pose , and combine the strengths of CNN and the cross-attention of transformer. Our proposed CTA-Depth block allows global processing of scene information and yields a more robust and accurate prediction, even for moving objects as well as messy environment.
